Pruning Redundant Mappings in Transformer Models via Spectral-Normalized Identity Prior

Traditional (unstructured) pruning methods for a Transformer model focus on regularizing the individual weights by penalizing them toward zero. In this work, we explore spectral-normalized identity priors (SNIP), a structured pruning approach that penalizes an entire residual module in a Transformer model toward an identity mapping. Our method identifies and discards unimportant non-linear mappings in the residual connections by applying a thresholding operator on the function norm. It is applicable to any structured module, including a single attention head, an entire attention block, or a feed-forward subnetwork. Furthermore, we introduce spectral normalization to stabilize the distribution of the post-activation values of the Transformer layers, further improving the pruning effectiveness of the proposed methodology. We conduct experiments with BERT on 5 GLUE benchmark tasks to demonstrate that SNIP achieves effective pruning results while maintaining comparable performance. Specifically, we improve the performance over the state-of-the-art by 0.5 to 1.0% on average at 50% compression ratio.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/final/01.new.introduction.tex <==
\section{Introduction}

Natural Language Processing (NLP) has recently achieved great success by using the Transformer-based pre-trained models \cite{radford2019language, devlin2018bert, yang2019xlnet, clark2020electra}. However, these models often consume considerable storage, memory bandwidth, and computational resource. To reduce the model size and increase the inference throughput, compression techniques such as knowledge distillation \cite{sanh2019distilbert, sun2019patient, tang2019distilling, jiao2019tinybert, sun2020mobilebert} and weight pruning \cite{guo2019reweighted, wang2019structured, gordon2020compressing, sanh2020movement} have recently been developed.

Knowledge distillation methods require the specification of a student network with a smaller architecture, which often has to be identified by a tedious sequence process of trial-and-error based decisions.
By comparison, the iterative pruning methods gradually prune the redundant model weights or layers from the full-size model, and provide a full picture of the trade-off between the task performance and the model size with a single training process, as illustrated in Figure \ref{fig:example}. This allows the iterative pruning methods to easily determine the most compact architecture given a required level of model performance.

\begin{figure}[t]
    \centering
    \includegraphics[width=7.5cm]{images/others/mnli_prune.pdf}
    \caption{Comparison of selected knowledge distillation methods (DistilBERT \cite{sanh2019distilbert} and BERT-PKD \cite{sun2019patient}) and iterative pruning methods (Iterative Pruning \cite{guo2019reweighted} and our proposed method) in terms of accuracy at various compression rate using MNLI test set. knowledge distillation methods require re-distillation from the teacher to get each single data point, whereas iterative pruning methods can produce continuous curves at once.}
    \label{fig:example}
\end{figure}

However, many of the existing pruning methods rely on classic regularizers that act on the individual weights by penalizing them to zero \cite{guo2019reweighted, sanh2020movement}. As a result, the pruned model tends to maintain the same architecture as the original model despite the reduced parameter count, which does not practically lead to an improvement in inference latency \cite{wen2016learning}.

This leads to a question: is it possible to perform more structured pruning on a Transformer model to modify its model architecture (e.g., reducing width and depth)?

To this end, we notice that many previous works have suggested that the learned Transformer models often have much redundancy \cite{tenney2019bert, liu2019linguistic, jawahar2019does, kovaleva2019revealing}. For example, \citet{michel2019sixteen, voita2019analyzing} found that most of the attention heads in a Transformer model can be removed without significantly impacting accuracy, and \citet{tenney2019bert} found that while the earlier layers and the later layers in a BERT model play clear roles in extracting either low-level or task-specific linguistic knowledge, the roles of the intermediate layers are less important. These observations have motivated the idea that Transformer models may exhibit considerable \textit{structural redundancy} - i.e., some layers can be removed during the training without harming the final performance.

In this paper, we propose a \emph{structured} pruning method that reduces the architecture of a Transformer by directly targeting its sub-modules as a whole - for example, a single attention head, an attention module, a feed-forward subnetwork, etc.
We take an approach we call \textit{spectral-normalized identity prior} (SNIP), which imposes a function-level prior centered around the identity function on the aforementioned modules.

Specifically, we take the advantage of the residual blocks ($\mathcal{F}(x) + x$) within a Transformer layer and compress them to \emph{strict identity mappings} \cite{yu2018learning} by identifying the residual blocks whose nonlinear mapping's absolute values ($|\mathcal{F}(x)|$) mostly fall below a threshold $\epsilon$. 
With this strategy, the weights of the Transformer model can still be under-regularized when using simple $L_1$ or $L_2$ based regularizers, which cause the distribution of the post-activation values prone to be noisy even after layer normalization \cite{ba2016layer}.
To address this issue, we further leverage \emph{spectral normalization} \cite{miyato2018spectral} to stabilize the distribution of the post-activation values by regularizing the largest singular value of the weight matrices.

We use BERT \cite{devlin2018bert} as a case study in this paper.
Across multuple tasks in the GLUE benchmark \cite{wang2018glue}, SNIP improves the performance over the state-of-the-art by $0.5$ to $1.0\%$ on average at 50\% compression ratio. \footnote{Open-source code can be found at \url{https://github.com/google-research/google-research/tree/master/snip}}
We also show that spectral normalization results in more sparse and regulated layer mappings during pre-training.
We compare the remaining model components across the tasks at a fixed compression ratio in an ablation study, and show that the remaining components are similar but not identical.

Our contributions are three-fold: First, we introduce \textit{identity-inducing prior}, a structured pruning approach that imposes identity-inducing regularization on the Transformer mappings as a whole rather than its individual weights.
%This approach iteratively identifies an ideal architecture and practically achieves inference speedup.
Second, we show that through a novel combination with the \textit{spectral normalization} regularization, the resulting \textit{spectral-normalized identity prior} (SNIP) leads to well-regularized weight distribution and sparse layer mappings in a BERT model. 
Finally, we conduct thorough experiments to validate the SNIP approach over 5 standard NLU tasks. Our results suggest that different model components in a Transformer play critically different roles across tasks, suggesting the importance of performing task-specific pruning to obtain an architecture that is the most suitable for the target task.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/final/02.new.related_work.tex <==
\section{Related Work}
\paragraph{Pre-trained Language Model Compression}
The major existing efforts to compress pre-trained language models such as BERT include knowledge distillation \cite{ba2014deep, hinton2015distilling} and pruning \citep{iandola2016squeezenet, veit2017convolutional}.

The knowledge distillation approach enables the transfer of knowledge from a large \textit{teacher} model to a smaller \textit{student} model. Such attempts have been made to distill BERT models, e.g., DistilBERT \cite{sanh2019distilbert}, BERT-PKD \cite{sun2019patient}, Distilled BiLSTM \cite{tang2019distilling}, TinyBERT \cite{jiao2019tinybert}, MobileBERT \cite{sun2020mobilebert}, etc.
All of these methods require carefully designing the student architecture. Furthermore, to choose which intermediate results that the student model can learn from, e.g., the outputs of each layer, the attention maps, is still under discussion.

Similar to other pruning-based methods, our method can iteratively remove the least important weights or connections, explore the full spectrum of trade-offs, and find the best affordable architecture in one shot.

Many language representation model pruning methods focus on individual components of the weight matrices. For example, \citet{guo2019reweighted} integrates reweighted $L_1$ minimization with a proximal algorithm to search sparsity patterns in the model; \citet{gordon2020compressing} uses magnitude weight pruning, which compresses the model by removing weights close to 0; \citet{sanh2020movement} applies deterministic first-order weight pruning method where both weights with low and high values can be pruned. A very few works try structured weight pruning, e.g., \citet{wang2019structured} proposes a structured pruning approach based on low-rank factorization and augmented Lagrangian $L_0$ norm regularization. On the other hand, there also exist works that prune a coherent set of sub-modules in the Transformer model. For example, 
\citet{michel2019sixteen} and \citet{voita2019analyzing} propose to prune individual attention heads either manually via head importance score, or automatically via a relaxed $L_0$ regularization. \citet{fan_reducing_2020} applies random pruning to the entire layers. In contrast, our method allows finer-grained structured pruning on Transformer modules (i.e., both attention heads and feed-forward layers) and propose to improve the mathematical property of a Transformer (i.e., Lipschitz condition) for more effective pruning.

Other compression approaches include weight sharing \cite{liu2019roberta}, quantization \cite{zafrir2019q8bert, shen2019q} and neural architecture search \cite{chen2020adabert}, but are not within the discussion of this paper. We refer interested readers to \citet{ganesh2020compressing} for further details.

\paragraph{Applications of Spectral Normalization}

Spectral normalization is first proposed for generative adversarial network (GAN) as a regularization technique to stabilize the discriminator training \citep{miyato2018spectral}. It was later applied to improve the performance of the other types of generative neural networks \citep{zhao_adversarially_2018, behrmann_invertible_2019}, and was analyzed theoretically in the context of adversarial robustness and generalization \citep{farnia_generalizable_2018}.

Spectral normalization regularizes the Lipschitz condition of the model mappings and is known to benefit model generalization under both the classic and the adversarial settings \citep{sokolic2017robust, cisse2017parseval, oberman2018lipschitz, neyshabur2017exploring}. In this paper, we will explore the benefit of spectral regularization for improving the effectiveness of pruning.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/final/03.new.method.tex <==
\section{Methods}

In this section, we first briefly review the basic Transformer layers in \citet{vaswani2017attention} (\ref{sec:background}). We then introduce our identity prior into Transformer's residual connections using $\epsilon$ threshold (\ref{sec:identity_mapping}). In section \ref{sec:sepctral-normalization}, we give mathematical foundations to the spectral normalization and show how it could help with our identity prior. Finally, to put it all together, we establish our structured iterative pruning methods for BERT fine-tuning (\ref{sec:iterative-pruning}).

\subsection{Background: Transformer Layer}
\label{sec:background}
Transformer-based models are usually comprised of a stack of Transformer layers. A Transformer layer takes on a sequence of vectors as input, first passes it through a (multi-head) self-attention sub-layer, followed by a position-wise feed-forward network sub-layer.

\paragraph{Self-attention sub-layer}
The attention mechanism can be formulated as querying a dictionary with key-value pairs. Formally, 
\begin{align*}
    \textrm{Att}(Q, K, V)=\textrm{softmax}(QK^T/\sqrt{d_H}) \cdot V
\end{align*}
where $d_H$ is the dimension of the hidden representations. $Q$, $K$, and $V$ represent query, key, and value. The multi-head variant of attention (MHA) allows the model to jointly attend to information from different representation sub-spaces, defined as
\begin{align*}
    \textrm{MHA}(Q, K, V) &= [\textrm{head}_1, \ldots, \textrm{head}_A] W^O \\
     \textrm{head}_k &= \textrm{Att}(QW_k^Q, KW_k^K, VW_k^V)  
\end{align*}

\noindent where $[\cdot,\cdot]$ is the concatenation operator, $W_k^Q\in \mathbb{R}^{d_H \times d_K}$, $W_k^K\in \mathbb{R}^{d_H\times d_K}$, $W_k^V\in \mathbb{R}^{d_H\times d_V},$ and $W^O\in \mathbb{R}^{Hd_V \times d_H}$ are projection parameter matrices, $A$ is the number of heads, and $d_K$ and $d_V$ are the dimensions of key and value. 

\paragraph{Position-wise FFN sub-layer}
In addition to the self-attention sub-layer, each Transformer layer also contains a fully connected feed-forward network, which is applied to each position separately and identically. This feed-forward network consists of two linear transformations with an activation function $\sigma$ in between. Specially, given vectors $\mathbf{x}_1, \ldots, \mathbf{x}_n$, a position-wise FFN sub-layer transforms each $\mathbf{x}_i$ as $\text{FFN}(\mathbf{x}_i) = \sigma(\mathbf{x}_iW_1+b_1) W_2 + b_2$, where $W_1, W_2, b_1$ and $b_2$ are parameters.

We should also emphasize that a residual connection \cite{he2016identity} and a layer normalization \cite{ba2016layer} are applied to the output of both MHA or FNN sub-layers. The residual connection plays a key role in learning strict identity mapping (detailed in Section \ref{sec:identity_mapping}), while layer normalization and spectral normalization (detailed in Section \ref{sec:sepctral-normalization}) together ensure regulated magnitude of activation outputs for improved pruning stability.

\subsection{Identity-inducing Prior for Transformer}
\label{sec:identity_mapping}

The design of residual connection can provide us with a promising way to find identity mappings for the Transformer model. Specifically, residual connection \cite{he2016identity} can be formalized as $\mathcal{H}(\mathbf{x}) = \mathcal{F}(\mathbf{x}) + \mathbf{x}$, where $\mathcal{F}$ could be either $\textrm{MHA}$ or $\textrm{FFN}$ and $\mathcal{H}$ is the sub-layer output.
As illustrated in \citet{he2016deep}, if an identity mapping is optimal, it is easier to push the residual to zero than to fit an identity mapping by a stack of traditional non-linear layers.

We leverage $\epsilon$-ResNet \cite{yu2018learning}, a strict identity mapping mechanism that sparsifies the layer output by inducing a specific threshold $\epsilon$ as the \textit{identity prior}.
Specifically, we turn the residual connection $\mathcal{H}(\mathbf{x})$ into $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) + \mathbf{x}$, where 
\begin{equation*}
\mathcal{S}_\epsilon(\mathbf{v}) = 
\left\{
\begin{array}{ll}
    0 &  \textrm{if } |\mathbf{v}_i|<\epsilon, \forall i \in {1, ..., |\mathbf{v}|},\\
    \mathbf{v} & \textrm{otherwise,}
\end{array}
\right.
\end{equation*}

\noindent where $\mathbf{v}_i$ is the $i$-th element of the vector $\mathbf{v}$.
Here a sparsity-promoting function $\mathcal{S}$ is applied to dynamically discard the non-linearity term based on the activations. When all the responses in the non-linear mapping $\mathcal{F}(\mathbf{x})$ is below a threshold $\epsilon$, then $\mathcal{S}(\mathcal{F}(\mathbf{x}))=0$, otherwise, the original mapping $\mathcal{S}(\mathcal{F}(\mathbf{x}))=\mathcal{F}(\mathbf{x})$ was used as the standard residual network.

To implement $\mathcal{S}$, we put an extra binary gate layer $t_\epsilon$ upon $\mathcal{F}(\mathbf{x})$ by stacking additional rectified linear units (ReLU), following \citet{srivastava2015highway}. In particular,
\begin{equation*}
    t_\epsilon (\mathbf{v}) = 1 - \textrm{ReLU}(1-L \max\limits_{1 \le i \le |\mathbf{v}|}\textrm{ReLU}(|\mathbf{v}_i| - \epsilon))
\end{equation*}

\noindent where $L$ refers to a very large positive constant (e.g., $1e5$ in our experiments). Then, $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{v}))$ has the following form:
\begin{equation*}
    \mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) = t_\epsilon (\mathcal{F}(\mathbf{x})) \mathcal{F}(\mathbf{x})
\end{equation*}

Recall that each layer of Transformer consists of two residual blocks, namely, the self-attention sub-layer and the position-wise FFN sub-layer. We apply the $\epsilon$ network directly to the residual block in the FFN sub-layer, i.e., 
\begin{align*}
    \mathcal{H}_\textrm{FFN}(\mathbf{x}) = \mathcal{S}_{\epsilon_\textrm{FFN}}(\textrm{FFN}(\mathbf{x})) + \mathbf{x},
\end{align*}

\noindent When applying it to the attention sub-layer, we place $\mathcal{S}$ to each single attention head, which allows us to prune any subset of attention heads, i.e., 
\begin{align*}
    \mathcal{H}_\textrm{ATT}(\mathbf{x}) = \sum_{i=1}^A \mathcal{S}_{\epsilon_\textrm{ATT}}(\textrm{head}_i W^O_i) + \mathbf{x}
\end{align*}

\noindent Here, $W^O_i$ is the output weight assign to the $i$-th attention head, i.e., $W^O=[W^O_I, W^O_2, ..., W^O_A]$. If $\mathcal{S}_{\epsilon_\textrm{ATT}}(\textrm{head}_i W^O_i) = 0$, this means that the $i$-th attention head does not contribute to the output of the attention layer and thus could be pruned out.

In our experiment, we set different values to $\epsilon_\textrm{ATT}$ and $\epsilon_\textrm{FFN}$, since the absolute outputs of attention and FFN layers lay in different scalars, as illustrated in Figure \ref{fig:output-distribution}.

\begin{figure*}[tb]
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/final/att_output_distibution.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/final/ffn_output_distibution.pdf}
    \end{minipage}
    \\
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/final/att_output_distibution_norm=5.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/final/ffn_output_distibution_norm=5.pdf}
    \end{minipage}
    \caption{Distribution of the max absolute value of the attention/FFN outputs on the Stanford Sentiment Treebank (SST) training set, based on model BERT$_\textrm{BASE}$ (w/o SN) and spectral normalized BERT$_\textrm{BASE}$ (w/ SN). For attention layers, different heads are plotted separately but with the same color in the same layer for clarity. After SN, the norm distribution $P(|\mathcal{F}_k(\mathbf{x})|)$ shows a better separation (bottom v.s. top), and the norms distribution for the FFN layers are stabilized within a much smaller range (bottom right v.s. top right).}
    \label{fig:output-distribution}
\end{figure*}

\subsection{Spectral Normalization}
\label{sec:sepctral-normalization}

The sparsity-inducing function $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x}))$ in the $\epsilon$-ResNet has been found to work well for randomly initialized neural network, where the initial weight matrix of the non-linear mappings for all layers was distributed within a consistent range, and thus facilitates a natural separation between the function norms $|\mathcal{F}|$ of the important and unimportant non-linear mappings in the residual blocks during training \citep{yu2018learning}. This is, however, not the case for the weight distribution of a pre-trainined model like BERT, where the weight distributions between different layers have already diverged during pre-training, which is likely due to the specialization of layer functionalities under the masked language modeling (MLM) training \citep{tenney2019bert}.

\begin{table}[tb]
    \centering\scalebox{0.8}{
    \begin{tabular}{lcccccc}
    \toprule
        \textbf{SN}                  & \textbf{MLM} & \textbf{SST-2} & \textbf{QQP} & \textbf{MRPC} & \textbf{QNLI} & \textbf{MNLI}\\\midrule
        w/o                & 71.93       & 92.7        & 90.6        & 90.9         & 91.6         & 84.7           \\
        % BERT$_\textrm{BASE}$ ($\sigma(W)=1$) & 70.72       & 90.4        & 89.0        & 89.2         & 89.0         & 80.6           \\
        % BERT$_\textrm{BASE}$ ($\sigma(W)=2$) & 73.43       & 91.3        & 90.1        & 90.3         & 91.5         & 84.0           \\
        w/ & 74.16       & 91.9        & 90.1        & 90.8         & 91.6         & 85.1           \\
    \bottomrule
    \end{tabular}}
    \caption{Evaluate the performance of BERT$_\textrm{BASE}$ (w/o SN) and the spectral normalized BERT$_\textrm{BASE}$ (w/ SN, using $\lambda(W)=5$), respectively masked language modeling accuracy on pre-training data and accuracy of fine-tuning on 5 natural language understanding tasks (details could be found in Section \ref{sec:datasets}).
    }
    \label{tab:performance-on-different-norm}
\end{table}

Indeed, in our preliminary experiments, we observed that the proposed identity-inducing prior $\epsilon$ is not effective for a BERT model initialized from a classic pre-training checkpoint. As shown in Table \ref{tab:performance-on-different-norm}, we found the distribution of the function norms $P(|F(\mathbf{x})_i|)$ for the attention layers to be densely clustered within a small range ($(0, 2)$) and with no clear separation between the function norm for the important and unimportant non-linear residual mappings. On the other hand, the norm distributions for different FFN layers were found to vary wildly, creating challenges for selecting a proper set of $\epsilon$'s in practice.

The above observations motivate us to identify an effective method to stabilize the norm distributions of BERT model layers. In this work, we consider \textit{spectral normalization} (SN), an approach that directly controls the Lipschitz norm of a non-linear mapping $\mathcal{F}$ by regularizing the spectral behavior of its weight matrices \citep{miyato2018spectral}. 

Specifically, for a weight matrix $W$, its spectral norm $\lambda(W)$ is defined as its largest singular value:
\begin{align*}
    \lambda(W) = 
    \underset{x\neq0}{\textrm{max}}\frac{||W\mathbf{x}||_2}{||\mathbf{x}||_2}.
\end{align*}

\noindent We say a function $\mathcal{F}$ is $L$-Lipschitz if $|\mathcal{F}(\mathbf{x}_1)-\mathcal{F}(\mathbf{x}_2)|/||\mathbf{x}_1 - \mathbf{x}_2|| \leq L$, for all possible $(\mathbf{x}_1, \mathbf{x}_2)$ pairs from the feature space, and we call the smallest possible $L$ the Lipschitz norm of $\mathcal{F}$, denoted as $|\mathcal{F}|_{Lip}$. 
Consequently, for a neural network mapping $\mathcal{F}(\mathbf{x}) = \sigma(W\mathbf{x} + b)$ with an contractive activation function $\sigma$,
its Lipschitz norm is upper-bounded by $\lambda(W)$ \citep{miyato2018spectral}:
\begin{equation*}
    |\mathcal{F}|_{Lip} = |\sigma(W \mathbf{x} + b)|_{Lip} \leq |W \mathbf{x} + b|_{Lip} \leq \lambda(W).
\end{equation*}

For BERT models, since the layer input $\mathbf{x}$ follows a  distribution of zero mean and unit variance due to layer normalization \cite{ba2016layer}, a nonlinear mapping's $L_1$ norm $|\mathcal{F}|$ is roughly proportional to its Lipschitz norm $|\mathcal{F}|_{Lip}$, which is controlled by $\lambda(W)$.
Therefore, we are able to have a better control of the maximum of $|\mathcal{F}(\mathbf{x})|$ for identifying a good $\epsilon$. Furthermore, the regularization is achieved by that the layer weights are simply divided by their corresponding spectral norm in SN, i.e., $\hat{W} = W / \hat{\lambda}(W)$, adding no additional trainable parameter to the original model.

\begin{figure*}[tb]
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/sst.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/qqp.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/mrpc.pdf}
    \end{minipage}%
    \\
    \begin{minipage}[t]{0.5\textwidth}
        \includegraphics[width=5.5cm, right]{images/performance/qnli.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \includegraphics[width=5.5cm, left]{images/performance/mnli.pdf}
    \end{minipage}
\caption{Evolution of performance when separately pruning attention heads (ATT) and FFN layers (FFN), and joint pruning ATT and FFN (Joint) on 5 GLUE dev sets. * means applying spectral normalization. The percentage pruned (x-axis) is calculated based on the parameters of attention and FFN sub-layers as the full set (excluding embedding, pooler and classifier layers). Joint pruning with spectral normalization (Joint*) could prune more parameters than the original BERT (Joint) to preserve the same accuracy.}
\label{fig:results}
\end{figure*}

We apply SN to both pre-training and fine-tuning of the BERT model, and on the weights in both the attention and the FFN layers. As shown in Table \ref{tab:performance-on-different-norm}, compared to the original BERT$_\textrm{BASE}$ without SN, adding SN to a BERT$_\textrm{BASE}$ model has resulted in improved pre-training performance and competitive fine-tuning performance. To illustrate the effect of SN on the distribution of function norms of the BERT model, we plot $|\mathcal{F}(\mathbf{x})|$ for the training set of the Stanford Sentiment Treebank in Figure \ref{fig:output-distribution}. As shown, after SN, the norm distribution $P(|\mathcal{F}_k(\mathbf{x})|)$ between the important and the unimportant nonlinear mappings shows a better separation (Figure \ref{fig:output-distribution}, bottom), the norms distribution for the FFN layers are now stabilized within a much smaller range (Figure \ref{fig:output-distribution}, bottom right).

\subsection{Structured Iterative Pruning}
\label{sec:iterative-pruning}
% The choice of $\epsilon_\textrm{ATT}$ and $\epsilon_\textrm{FFN}$ can be regulated by some prior distribution and optimized during training.\todo{What does it mean?} 
We use a simple pruning method that greedily and iteratively prunes away attention heads and FFN layers to avoid impractical combinatorial search, where two dynamic estimations are conducted for $\epsilon$ and model architecture respectively.
%given the number of attention heads and the time it takes to evaluate each model.
One iteration contains four substeps: 
\begin{enumerate}
    \item Estimate $\epsilon$ given current model architecture and training data. Specifically, %evaluate the output distribution and determine $\epsilon$. 
    % Note that in this case, a better distribution could help us get better control of $\epsilon$.
    % As $\epsilon$ satisfies a nice monotonicity property --- 
    % Larger $\epsilon$ leads to higher compression.
    % We could start from a relatively low $\epsilon$ and gradually increase it at each iteration to achieve a higher compression rate.
    We sort the attention heads and FFN layers by their mean activation outputs, and set $\epsilon$ to the $k$-th smallest mean activation.
    Larger $k$ leads to more mappings being pruned in one iteration, which makes the retraining more difficult to recover the performance, but leads to fewer pruning iterations.
    
    \item Train the model with identity-inducing prior by using the selected $\epsilon$.
    
    \item Estimate a smaller architecture given current $\epsilon$ and training data.
    Specifically, we estimate the module usage by counting the number of times each residual block has been learned to become a strict identity mapping across mini-batches in the training set.
    We prune residual blocks whose usage rate below a threshold $\theta$.
    When a residual block produces a negligible response, the $\epsilon$ function will start producing $0$ outputs. As a result, the weights in this block will stop contributing to the cross-entropy term. Consequently, the gradients will only be based on the regularization term and lead to weight collapse.
    
    \item Retrain the model with the pruned residual blocks completely removed from the architecture.
    This is critical --- if the pruned network is used without retraining, accuracy is significantly impacted. 
    Also, during retraining, it is better to retain the weights from the initial training phase for the connections that survived pruning than it is to re-initialize them \cite{han2015learning}.
\end{enumerate}

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/final/04.new.experiments.tex <==
\begin{table*}[tb]
    \centering
    \scalebox{0.76}{
    \begin{tabular}{lrccccc}
    \toprule
        \textbf{Model}                            & \textbf{FLOPS} & \textbf{ SST-2$_{acc}$} & \textbf{QQP$_{acc}$} & \textbf{MRPC$_{F_1}$} & \textbf{QNLI$_{acc}$} & \textbf{MNLI-mm$_{acc}$}\\\hline
        BERT$_\textrm{BASE}$                      & 22.5B          & \ \ -0.0\%/92.7        & \ \ -0.0\%/90.6       & \ \ -0.0\%/90.9        & \ \ -0.0\%/91.6        & \ \ -0.0\%/84.7 \\
        TinyBERT$_6$ w/o DA \cite{jiao2019tinybert}\protect\footnotemark & 1.2B         & -                      & -                     & -50.0\%/86.0           & -                      & \textbf{-50.0\%/84.4}\\
        DistilBERT$_6$ \cite{sanh2019distilbert} & 11.3B          & -50.0\%/91.3           & -50.0\%/88.5          & -50.0\%/87.5           & -50.0\%/89.2           & -50.0\%/82.2 \\
        BERT-PKD$_6$ \cite{sun2019patient}        & 11.3B          & -50.0\%/91.5           & \textbf{-50.0\%/88.9}          & -50.0\%/86.2           & -50.0\%/89.0           & -50.0\%/81.0 \\
        BERT-PKD$_3$ \cite{sun2019patient}        & 7.6B           & -75.0\%/87.5           & -75.0\%/87.8          & -75.0\%/80.7           & -75.0\%/84.7           & -75.0\%/76.3 \\
        \hline
        FLOP \cite{wang2019structured}           & 15B             & -35.0\%/92.1           & -                     & -35.0\%/88.6           & -35.0\%/89.0           & -           \\
        MvP \cite{sanh2020movement} $\dagger$    & N/A             & -                      & -97.0\%/89.2          & -                      & -                      & -97.0\%/79.7\\\hline\hline
        SNIP (w/ SN)          & 13.2 - 14.5B    & \textbf{-50.0\%/91.8}           & \textbf{-50.0\%/88.9}         & \textbf{-50.0\%/88.1}           & \textbf{-50.0\%/89.5}           & -50.0\%/82.8\\
        SNIP (w/ SN)          & 8.3 - 9.1B      & -75.0\%/88.4           & -75.0\%/87.8          & -75.0\%/81.2           & -75.0\%/84.6           & -75.0\%/78.3\\\hline
        SNIP (w/o SN)                          & 16.8 - 18.2B    & -30.0\%/91.3           & -38.7\%/89.5          & -39.7\%/89.9           & -26.1\%/90.8           & -32.3\%/83.5\\
        SNIP (w/ SN)          & 13.4 - 16.1B    & -56.7\%/91.7           & -40.7\%/89.7          & -46.7\%/89.9           & -36.0\%/90.7           & -39.3\%/83.9\\
    \bottomrule
    \end{tabular}}
    \caption{The compression results including model efficiency (percentage of reduced parameters) and performance from the GLUE dev results, and the MNLI result is evaluate for mismatched-accuracy (MNLI-mm). BERT$_\textrm{BASE}$ indicates the results of the fine-tuned BERT$_\textrm{BASE}$ in our implementation. The number of model parameters includes the attention and FFN sub-layers but excludes the embedding, pooler and classifier layers. The bold numbers indicate the best performance for keeping 50\% of the parameters respectively. Rows 1--5 are knowledge distillation methods, and Rows 6 and 7 are pruning methods, where $\dagger$ means unstructured pruning \protect\footnotemark.}
    \label{tab:best-architecture}
\end{table*}

\section{Experiments}

\subsection{Experimental Settings}
In the experiments, we apply the same architecture and the base settings from the original BERT$_\textrm{BASE}$ \cite{devlin2018bert}, and fine-tune each task independently. More details could be found in Appendix.
% \todo{weight based pruning baselines?}

% \subsection{Datasets}
\label{sec:datasets}
For pre-training, we use the same data as BERT, which consists of 3.3 Billion tokens from Wikipedia and BooksCorpus \citep{zhu2015aligning}. Similar to the standard BERT practice, we conduct the pre-training only once and from scratch (i.e., no second pre-training). We use dynamic token masking with the masked positions decided on-the-fly instead of during preprocessing. Also, we did not use the next sentence prediction objective proposed in the original BERT paper, as recent work has suggested it dost not improve the scores \cite{yang2019xlnet, liu2019roberta}.

For fine-tuning tasks, we focus on the General Language Understanding Evaluation (GLUE) benchmark \citep{wang2018glue} in the main text since it is a thoroughly studied setting in many pruning/distillation work, thereby allowing comprehensive comparison.
We conduct experiments on the subset of GLUE , classified into three categories:
\begin{enumerate}
    \item Sentiment analysis: Stanford Sentiment Treebank (SST) \cite{socher2013recursive};
    \item Paraphrasing: Quora Question Pairs (QQP) \cite{chen2018quora} and Microsoft Research Paraphrase Corpus (MRPC) \cite{dolan2005automatically};
    \item Natural language inference: Question Natural Language Inference (QNLI) \cite{chen2018quora}, and Multi-genre Natural Language Inference (MNLI) \cite{williams2017broad}. 
\end{enumerate}
The detailed description of downstream tasks could be found in Appendix. The reason for choosing this subset is that we found the variance in performance for those tasks lower than the other GLUE tasks. 

We used the hyperparameters from \citet{clark2020electra} for the most part. Since we run the training iteratively, we set train epoch as 1 for most of the task but 3 for task MRPC consider that the size of the datasets is much smaller than other tasks.

For $\epsilon$ and architecture estimations in Section \ref{sec:iterative-pruning}, we set $k=1$ and $\theta = 0.95$ in our experiment.

\begin{figure*}[tb]
    \centering
    \renewcommand{\arraystretch}{0}
    \begin{tabular}{p{0.005\textwidth}p{0.28\textwidth}p{0.28\textwidth}p{0.28\textwidth}}
            & \multicolumn{1}{c}{\ \ \ \ \ \ SST}   & \multicolumn{1}{c}{\ \ \ \ \ \ MRPC} &\multicolumn{1}{c}{\ \ \ \ \ \ MNLI} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 16.67\%} &  \includegraphics[width=0.33\textwidth]{images/ablation/sst/sst_iter1.pdf}    & \includegraphics[width=0.33\textwidth]{images/ablation/mrpc/mrpc_iter1.pdf} & \includegraphics[width=0.33\textwidth]{images/ablation/mnli/mnli_iter1.pdf} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 33.33\%} &  \includegraphics[width=0.33\textwidth]{images/ablation/sst/sst_iter2.pdf}    & \includegraphics[width=0.33\textwidth]{images/ablation/mrpc/mrpc_iter2.pdf} & \includegraphics[width=0.33\textwidth]{images/ablation/mnli/mnli_iter2.pdf} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 50.00\%} &  \includegraphics[width=0.33\textwidth]{images/ablation/sst/sst_iter3.pdf}    & \includegraphics[width=0.33\textwidth]{images/ablation/mrpc/mrpc_iter3.pdf} & \includegraphics[width=0.33\textwidth]{images/ablation/mnli/mnli_iter3.pdf}
    \end{tabular}
    \caption{
    Pruning map of attention heads (\texttt{att}) and FFN layers (\texttt{ffn}) during pruning on task SST-2, MRPC and MNLI dev sets. \texttt{mean} is the mean of attention heads of each layers. The left column shows the percentage of pruned parameters. Color white indicates that this attention head or FFN layer has been entirely pruned. For different tasks, the distribution of important attention heads is similar, but not identical, and certain FFN sub-layers might be more amenable to compression, even if the corresponding self-attention sub-unit is not.
    }
    \label{fig:heatmap}
\end{figure*}

\footnotetext[2]{TinyBERT \cite{jiao2019tinybert} utilizes data augmentation (DA), which makes it unfair to have a direct comparison. We only listed their results without DA.}
\footnotetext[3]{We do not list the results in \citet{guo2019reweighted, gordon2020compressing} since they show the results in scatter plots instead of the exact numbers, and similar to MvP \cite{sanh2020movement}, they are of unstructured pruning, which could not speed up the inference in practice.}

\subsection{Results}
We compare the pruning results on non-normalized and normalized BERT models on the 5 GLUE tasks, as shown in Figure \ref{fig:results}, which includes separate pruning for attention heads and FFN sub-layers and joint pruning of both modules. The results demonstrate the advantage of spectral normalization.

To put it all together, in Table \ref{tab:best-architecture}, we further show the simplest architecture we could get when allowed at most 1\% in terms of performance degradation. This also means that further slight pruning will have a noticeable impact on the final results. We find that spectral normalization can lead to a better trade-off between parameter size and performance. Specifically, for the same ideal performance shown in the last two rows in Table \ref{tab:best-architecture}, spectral normalized BERT could on average be pruned 12\% parameters more than the original BERT.

We also list other compression methods in the table for comparison while most of them are of knowledge distillation and have a pre-defined fixed size of the compressed model.
Our methods provide the flexibility to choose the best architecture and take advantage of finding the inflection point during pruning, while compared with other pruning methods we could practically speed up the inference time since we use a structured pruning.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/final/05.new.ablation_study.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=7.5cm]{images/ablation/ablation.pdf}
    \caption{Evolution of accuracy on the dev set of SST-2 for (1) pruning the whole attention layers (HA); (2) pruning single attention heads (MHA); (3) pruning the whole layer (Layer pruning) and (4) pruning the attention and FFN sub-layers separately (Separate pruning).}
    \label{fig:abaltion}
\end{figure}

\subsection{Analysis}
In this section, we investigate the contribution of: (1) single attention head pruning, and (2) split pruning for attention heads and FFN sub-layers.

\paragraph{Single Head Attention Pruning}

Multi-head self-attention is a key component of Transformer, where each attention head potentially focuses on different parts of the inputs. 

The analysis of multi-head attention and its importance is challenging. 
Previous analysis of multi-head attention considered the average of attention weights over all heads at given position or focused only on the maximum attention weights \cite{voita2018context, tang2018analysis}, or explicitly takes into account the varying importance of different heads \cite{voita2019analyzing}. 
\citet{michel2019sixteen} has proved that attention heads can be removed without significantly impacting performance, but they mainly focus on machine translation and NLI.

To understand whether and to what extent attention heads play consistent and interpretable roles when trained on different downstream tasks, we pick one task from the sentiment analysis, paraphrasing and natural language inference respectively, plot the pruned attention heads during training and show the dynamic process in Figure \ref{fig:heatmap}. We can find that though for different tasks, the distributions of important attention heads are similar, as reflected in the mean of each attention layer, the exact pruned attention heads are actually different. This also indicates that splitting the pruning for attention heads could have more flexibility for the model to find an optimal architecture.

\paragraph{Separate Pruning for Attention and FFN}

Decoupling and then individually studying the self-attention and the FFN sub-layers is important for understanding the progressive improvement they provide.
As can be observed from Figure \ref{fig:results}, for most of the tasks, pruning FFN layers damages the performance more than the attention layers, indicating that the compression technique for the Transformer model tends to be more effective on the attention layers \cite{voita2018context, michel2019sixteen}, than the FFN layers \cite{ganesh2020compressing}.

In Figure \ref{fig:heatmap}, similar to attention heads, we further plot the pruning map of FFN layers. We find that, certain FFN sub-layers might be more amenable to compression, even if the corresponding self-attention sub-unit is not. For example, in all the tasks, the FFN layers near the ends of input or output are more likely to be pruned, while this does not hold for the corresponding self-attention layers.

Finally, we compare between single head attention pruning and separate pruning for attention/FFN, and show the evolution of performance for single head attention pruning (HA), multi-head attention pruning (MHA), separate attention/FFN pruning, and whole layer pruning respectively in Figure \ref{fig:abaltion}. We find that MHA and separate pruning perform much better than HA and layer pruning.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/old/01.introduction.tex <==
\section{Introduction}


% \todo[color=green]{Dan: all the captions of the Figure and Table should stand alone without further reference on the text}
\begin{figure}[t]
    \centering
    \includegraphics[width=6.5cm]{images/others/mnli_prune.pdf}
    \caption{Comparison of selected knowledge distillation (KD) methods (DistilBERT \cite{sanh2019distilbert} and BERT-PKD \cite{sun2019patient}) and iterative pruning (IP) methods (Iterative Pruning \cite{guo2019reweighted} and our proposed method) in terms of accuracy at various compression rate using MNLI test set. KD methods require re-distillation from the teacher to get each single data point, whereas IP methods can produce continuous curves at once.}
    \label{fig:example}
    \vspace{-10pt}
\end{figure}

Natural Language Processing (NLP) has recently achieved great success by using the Transformer-based pre-trained models \cite{radford2019language, devlin2018bert, yang2019xlnet, clark2020electra}. However, these models often consume considerable storage, memory bandwidth, and computational resource. To reduce the model size and increase the inference throughput, compression techniques such as knowledge distillation \cite{sanh2019distilbert, sun2019patient, tang2019distilling, jiao2019tinybert, sun2020mobilebert} and weight pruning \cite{guo2019reweighted, wang2019structured, gordon2020compressing, sanh2020movement} have recently been developed. Knowledge distillation methods require a predefined fixed architecture (referred to as the \emph{student}) as a \emph{priori}, which often has to be identified by a tedious sequence process of trial-and-error. In comparison, iterative pruning methods gradually prune the redundant model weights or layers from the full-size model, and provides the full picture of the trade-off between the task performance and the model size with a single training process, as illustrated in Figure \ref{fig:example}.
% For example, in Figure \ref{fig:example} we show the performance on BERT fine-tuning task of iterative weight pruning \cite{guo2019reweighted}
% \todo[color=green]{This is not our method? And why the citation here is different from the one in the figure caption?}
% and two knowledge distillation methods \cite{sanh2019distilbert, sun2019patient}, where we can see that each performance point of knowledge distillation requires a trial of training, while pruning could provide the full image of the trade-off with a single training process, thus has more flexibility to find an optimal architecture.
%For instance, BERT \citep{devlin2018bert}, a widely-adopted pre-trained language representation model, has significantly improved the state-of-the-art across 11 different NLP tasks. However, these models consume considerable storage, memory bandwidth, and computational resource.

%It sometimes can only realistically be trained in large industrial research laboratories and such models trained with model parallelism cannot even be fine-tuned on a single GPU as their memory requirements demand a multi-accelerator hardware setup even for a single training step \citep{kitaev2020reformer}.

% To fulfill the deployment in real-time applications, many recent studies have been focused on making those giant models more efficient. Existing solutions include model parallelization \cite{} and model compression \cite{}. The former addresses the memory limitation problems, but not the communication overhead, while the latter aims to designing a lite version of the original architecture that has significantly fewer parameters.



% \todo[color=green]{Dan: perhaps add a figure show the difference of kd and wp, like Figure \ref{fig:abaltion}?}

% The former approach is ``bottom-up'', in the sense that it specifies a fixed architecture for the final compressed model as the priori. Based on this scenario, it is often loosely guided by a tedious sequence process of trial-and-error based decisions. Unlike knowledge distillation, weight pruning is ``top-down'', in the sense that it starts from the full size and prunes the redundancy in the weights/layers of the model.

Although iterative pruning methods make it easy to determine the most compact architecture given a required task performance, many focus on using sparsity-promoting regularizers to promote individual weight which can be arbitrary and usually irregular \cite{guo2019reweighted, sanh2020movement}. It actually cannot achieve superior runtime performance or even adversely impact practical acceleration in hardware platforms when compared with directly reducing numerical component modules \cite{wen2016learning}. On the other hand, previous works have questioned the importance of different component modules in the Transformer model and found that different components learn different levels of knowledge. For a specific downstream task, there are unimportant sub-modules focusing on knowledge not preferred by the task \cite{tenney2019bert, liu2019linguistic, jawahar2019does, kovaleva2019revealing}, i.e., those modules only provide relatively identical mappings that are not contributing to the final output. Therefore, we believe that these task-specific unimportant identity mappings could be identified and discarded by leveraging some \emph{identity priors}.

% \todo[color=green]{Can revive the pruning. Focus on the limitation of pruning.}
% \todo[color=green]{Briefly mention both distillation and pruning methods and explain them in the top-down/bottom-up way.}
% \todo[color=green]{also can mention that pruning is often regarded as a simpler compression method than distillation}

% \textbf{Discuss the unstructured and structured pruning: }For weight pruning, most of the previous works consider different sparsity-promoting regularization schemes for individual weights \cite{guo2019reweighted, sanh2020movement}. However, it often produces non-structured random connectivity and thus, irregular memory access that adversely impacts practical acceleration in hardware platforms \cite{wen2016learning}. %Furthermore, as illustrated in \citet{Brunner2020On}, there can be infinitely many different attention weights that yield the same output, thus the model redundancies are actually across different layers instead of only within each individual weights.

In this paper, we propose a \emph{structured} pruning method to prune higher-level mappings as a whole, e.g. a single attention head, an attention module, a feed-forward subnetwork, etc. in a Transformer-based model.
Specifically, we take the advantage of the residual blocks ($\mathcal{F}(x) + x$) of a Transformer layer and compress them to \emph{strict identity mappings} \cite{yu2018learning} by identifying the residual blocks whose nonlinearity activations ($\mathcal{F}(x)$) mostly fall below a threshold $\epsilon$.
% Specifically, the model will automatically discard redundant layers by learning \textit{strict identity mapping} \cite{yu2018learning} of the residual block, whose basic idea is that a ``useful'' layer should have magnitude above a certain threshold, so that we could discard those unimportant layers by ruling out those whose magnitudes are under the threshold. \textbf{In this way, the model could be more sparse at the level of layer mapping instead of individual weight.} 
% Several recent works have been focusing on large-scale pre-training models, among which a most widely-used technology is knowledge distillation \citep{hinton2015distilling}, where a compact model (the \textit{student}) is trained to reproduce the behavior of a larger model (the \textit{teacher}) or an ensemble of models \cite{sanh2019distilbert, sun2019patient, sun2020mobilebert, jiao2019tinybert}.
% While knowledge distillation has been proven to be a promising way to compress a large model into a small model, in the basic scenario, it requires the priori to pre-define the student's architecture, which is a tedious sequential process, often loosely guided by a sequence of trial-and-error based decisions to identify a smaller network architecture. This motivates us to develop a more principled approach to identifying optimal student architectures. 
% On the other hand, a model with smaller capacity can also be obtained by other model compression techniques such as sparsification, quantization, pruning and regularization, or even with their combinations, e.g., \citet{mishra2018apprentice} and \citet{polino2018model} are some works that combine knowledge distillation with quantization; \citet{theis2018faster} and \citet{ashok2018nn} combine distillation with pruning.
% In supervised learning, a classification model is generally trained to predict an instance class by maximizing the estimated probability of gold labels. A standard training objective thus involves minimizing the cross-entropy between the model's predicted distribution and the one-hot empirical distribution of training labels. A model performing well on the training set will predict an output distribution with high probability on the correct class and with near-zero probabilities on other classes. But some of these ``near-zero'' probabilities are larger than others and reflect, in part, the generalization capabilities of the model and how well it will perform on the test set. For example, the language representation model BERT \cite{devlin2018bert}'s predictions for a masked token in ``\texttt{I think this is the beginning of a beautiful [MASK]}'' comprise two high probability tokens (\textit{day} and \textit{life}) and a long tail of valid predictions (\textit{future, story, world}). 
% \todo[color=green]{lzi: the following three paragraphs seem to lose coherence}
However, the weight of the Transformer model could be still under-regularized when using simple $L_1$ or $L_2$ based regularizers, making the magnitude of the activation functions prone to be noisy even after layer normalization \cite{ba2016layer}.
% However, the problem of applying this approach to models like BERT is that, during task fine-tuning the weights are starting from pre-training, and the magnitude of the activation function is under-regularized, making the sparsity learning of fine-tuning less than guaranteed.
To address this issue, we further propose to leverage \emph{spectral normalization} \cite{miyato2018spectral} to restrict the largest singular value of the weight metrics in order to stabilize the magnitude (norm) of the activation functions.

While the proposed method could be applied to any Transformer-based network that has residual blocks, we use BERT \cite{devlin2018bert} as a case study in this paper.
We compare the performance of various compression methods across multiple tasks in the GLUE benchmark \citep{wang2018glue} and show that our proposed method improves the performance over the state-of-the-art by $+0.5 \sim 1.0\%$ on average at 50\% compression ratio.
% in paraphrsing, natural language inference and sentiment classification, where 
% we provide a clear task-dependent comparison on model complexity and their corresponding prediction performance, and achieve comparable results on some specific model sizes.
We also validate that by using spectral normalization, we could obtain more sparse and regulated layer mappings during BERT model pre-training, and compress to a model that can outperform the one pruned from the BERT model only with the ReLU activation function.
In the ablation study, we further compare the remaining model components across the tasks at the same compression ratio, and show that the remaining components are similar but not exactly identical.

% Another concern for the compression methodology is that whether we should have a task-agnostic or task-independent compressed model. As illustrated in previous work \cite{tenney2019bert, liu2019linguistic,jawahar2019does}, different layers of the model learn different levels of knowledge from the training data, while only certain part of the learned knowledge is needed for a specific downstream task. Therefore, different tasks theoretically should correspond to different model sizes, but what is the optimal structure combination and is this task-general still remain non-obvious. From an in-depth analysis of the pruning of separate model components, i.e., the attention and FFN sub-layers, we demonstrate that the redundancy components of the model are similar across different tasks but are not extremely identical. \todo{Motivate task-specific compression after introduction of model compression.}

% task-specific trade-off between computational complexity and prediction performance via structured sparse pruning on the attention heads and feed-forward functions in the Transformer model iteratively. 
% \todo{lzi: keyword: pruning - structured - mappings}
Our contributions are three-fold: First, we propose a structured pruning method applicable to mappings instead of individual weights,
which can iteratively identify an ideal architecture while practically achieve inference speedup.
Also, we novelly use spectural normalizated identity prior for BERT to obtain well-regularized weights and sparse layer mappings. 
Finally, we empirically show that on different downstream tasks, different model components play different critical roles, suggesting that we need to perform task-specific pruning to obtain different architectures.
% \todo[color=green]{Should this fact be observed by with some probing work also?}

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/old/02.related_work.tex <==
\section{Related Work}
\paragraph{Pre-trained Language Model Compression}
The major existing efforts to compress pre-trained language models such as BERT can be generally categorized into two lines: knowledge distillation \cite{ba2014deep, hinton2015distilling} and pruning \citep{iandola2016squeezenet, veit2017convolutional}. Other approaches include weight sharing \cite{liu2019roberta}, quantization \cite{zafrir2019q8bert, shen2019q} and neural architecture search \cite{chen2020adabert}, but are much more complicated and not within the discussion of this paper. \todo{lzi: might need to have a reason for skipping the discussion for other approaches?}

The knowledge distillation approach enables the transfer of knowledge from a large \textit{teacher} model to a smaller \textit{student} model, \textbf{which is improved in the process}. A line of works has been dealing with the knowledge distillation for the large-scaled Transformer-based model BERT, e.g., DistillBERT \cite{sanh2019distilbert}, BERT-PKD \cite{sun2019patient}, Distilled BiLSTM \cite{tang2019distilling}, TinyBERT \cite{jiao2019tinybert}, MobileBERT \cite{sun2020mobilebert}, etc.
However, state-of-the-art knowledge distillation methods share a common feature: they require carefully \textit{hand-designed} architectures for the student model, and this process makes it very difficult to explore the full spectrum of trade-offs and find the best affordable one. Furthermore, to choose which intermediate results that the student model can learn from, e.g., the outputs of each layers, the attention maps, are still under discussion.
% \todo{nhua: (it's confusing to me on "optimal", maybe) they require carefully \textit{hand-designed} architectures for the student model, and it's  difficult to explore the full spectrum of tradeoffs and find the best affordable. (Note that I doubt think this argument is strong enough while I can't do better)}

For pruning-based methods, the model is progressively removed, and therefore narrows the range of least important weight or connections. 
For language representation models, many of the existing work focus on unstructured or structured pruning of individual weights matrices. For example, \citet{guo2019reweighted} integrates reweighted $\textit{l}_1$ minimization with a proximal algorithm to search sparsity patterns in the model; \citet{wang2019structured} proposes a structured pruning approach based on low-rank factorization and augmented Lagrangian $\textit{l}_0$ norm regularization; \citet{gordon2020compressing} uses magnitude weight pruning, which compresses the model by removing weights close to 0; \citet{sanh2020movement} applies deterministic first-order weight pruning method where both weights with low and high values can be pruned. On the other hand, within the context of the transformer model, there also exists work that focuses on pruning a coherent set of sub-modules. The examples include 
\citet{michel2019sixteen} and \citet{voita2019analyzing} that prunes individual attention heads either manually via certain head importance score, or automatically via a relaxed $L_0$ regularization, and also \citet{fan_reducing_2020} that applies random pruning to the entire layers. Our work differs from these approaches in that we consider a principled pruning strategy that allows fine-grained pruning on all transformer modules (i.e., both the attention heads and the feed-forward layers), and we study the benefit of improving the mathematical property of a transformer (i.e. Lipschitz condition) to the effectiveness of pruning.
% \todo[color=white]{\jzl{below statements are a bit strong since there do exist module /  layer-wise pruning approaches. I added few sentences about module-wise/layer-wise approaches above , PTAL. }}
%\textbf{However, these works focus on either unstructured or structured pruning on the individual weight matrices, while none has tried a more structured way to prune at the layer level.} \todo{What is the disadvantage of those works? Why should we try pruning at layer / function / activation level?} \todo{LayerDrop?}
% \todo[color=green]{Is the focus to compare weight based vs activation based?}

% There are many work dealing with the model 
% BERT \cite{devlin2018bert} is a Transformer model pre-trained on large corpora using two training objectives: Masked Language Model (MLM), which helps it learn the context in a sentence, and Next Sentence Prediction (NSP), where it learns the relationship between two sentences. Transformer-based models can be compressed using low-rank approximation, weight sharing, knowledge distillation, quantization, or pruning.

% \paragraph{Language Representation Models} Learning representations of natural language has been shown to be useful for a wide range of NLP tasks and has been widely adopted \cite{mikolov2013distributed, dai2015semi, peters2018deep, devlin2018bert, radford2019language}.
% One of the most significant changes in the last two years is the shift from pre-training word embeddings, whether standard \cite{mikolov2013distributed, pennington2014glove} or contextualized \cite{mccann2017learned, peters2018deep}, to full-network pre-training followed by task-specific fine-tuning \cite{dai2015semi, radford2019language, devlin2018bert}. 

% The most well-known example is BERT \cite{devlin2018bert}, a Transformer model pre-trained on large corpora using two training objectives: Masked Language Model (MLM), which helps it learn the context in a sentence, and Next Sentence Prediction (NSP), where it learns the relationship between two sentences. Other Transformer-based pre-trained models includes GPT-2 \cite{radford2019language}, XLNet \cite{yang2019xlnet}, ELECTRA \cite{clark2020electra}, T5 \cite{raffel2019exploring}, etc.

% However, those most recently Transformer-based models often have over billion parameters, which can be prohibitively costly. This problem is exacerbated when we consider devices with lower capacity, e.g., smartphones, and applications with strict latency constraints, e.g., interactive chatbots or search engine. Therefore, efficient methods for compressing those models are desperately in need.\todo{I would probably discard this subsection. Instead, add a preliminary subsection at the beginning of next section to review BERT architecture.}


% To achieve this goal for the Transformer-based model, many works consider leveraging different sparse-promoting regularization schemes, e.g., $\textit{l}_0$ regularization \cite{voita2019analyzing, wang2019structured}, (reweighted) $\textit{l}_1$ regularization \cite{guo2019reweighted}. 
% A prominent line of work is devoted to compressing large neural networks to accelerate inference. Early pioneering works mainly targeted on convolutional neural networks (CNNs) \citep{lecun1990optimal, han2015deep, li2016pruning, liu2017learning, tang2018flops, chen2018constraint, wu2018training}, while many actually could be applicable to Transformers. Common techniques include (1) quantization, which uses fewer bits to represent the parameters, e.g., \citet{hubara2017quantized}, \citet{zafrir2019q8bert}, and \citet{shen2019q}; (2) pruning, which removes less important parameters, including sparse pruning that focuses on locating the set of least important weights in the model \citep{guo2019reweighted, gordon2020compressing}, and structured pruning that focuses on pruning the architectural components \cite{kovaleva2019revealing, michel2019sixteen, raganato2020fixed}; (3) parameter sharing across similar model units \cite{lan2019albert}.

% Other work tries to apply a differentiable neural architecture search for the original models \cite{chen2020adabert}.

% \paragraph{Strict Identity Mapping}
% In this paper, we introduce strict identity mapping, or residual pruning into the Transformer model, which was originally proposed by \cite{yu2018learning} and used in ResNet \cite{he2016deep}.

%Therefore, towards a more principled approach to network architecture compression, many works have been trying to combine traditional compression with knowledge distillation \cite{mishra2018apprentice, polino2018model, theis2018faster, ashok2018nn}, but very few works deal with the transformer model.


% Typical approaches include (1) sparse decomposition \cite{liu2015sparse}; (2) sparsity regularizer \cite{alvarez2016learning, wen2016learning}, which defines a group sparsity regularizer on the parameters of the network; (3) weight elimination \cite{han2015deep, han2015learning}, which learns the sparsity pattern of network weights by eliminating weight whose absolute value is less than an empirical threshold; (4) strict identity mapping \cite{yu2018learning}.

% \paragraph{Invertible Network} Invertible Network, first introduced in \cite{gomez2017reversible}, could address the issue of memory consumption when training a giant model. As one needs to store the activations in order to calculate gradients using backpropagation, making the network invertible allows us to reconstruct each layer's activations exactly from the next layer's, resulting in freeing the memory of the activations for most layers. Recently, a line of works begin to develop invertible variants \cite{gomez2017reversible, jacobsen2018revnet, behrmann2018invertible, kitaev2020reformer} of widely-used deep learning models such as ResNet \cite{he2016deep} and Transformer \cite{vaswani2017attention}. Typically, enforcing invertibility requires partitioning dimensions or modifying network architectures and negligible performance change need to be pre-guaranteed \cite{gomez2017reversible, jacobsen2018revnet, kitaev2020reformer}. Recently, \cite{behrmann2018invertible} showed that standard ResNet architectures can be made invertible by adding a simple normalization in standard frameworks. We will further introduce this normalization in Section \ref{ref:sepctral-normalization}.


\paragraph{Applications of Spectral Normalization}
%\todo{Add subsection to residual pruning and spectral norm}

Spectral normalization is first proposed for generative adversarial network (GAN)  
as a regularization technique to stabilize the discriminator training \citep{miyato2018spectral}. It was later applied to improve the performance of the other types of generative neural networks \citep{zhao_adversarially_2018, behrmann_invertible_2019}, and was analyzed theoretically in the context of adversarial robustness and generalization \citep{farnia_generalizable_2018}. In this paper, we will explore the benefit of spectral regularization for improving the effectiveness of pruning.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/old/03.method.tex <==
\section{Method}

% In this section, we will lay the theoretical groundwork for our proposed method.
In this section, we describe in the detail the proposed iterative mapping pruning method.

\subsection{Background: Transformer Layer}
Transformer-based models are usually comprised of a stack of Transformer layers. A Transformer layer takes on a sequence of vectors as input, first passes it through a (multi-head) self-attention sub-layer, followed by a position-wise feed-forward network sub-layer.%\textbf{ It outputs a new sequence of vectors of the same shape.}
% The computation inside a layer is decomposed into two steps: the vector first pass through a (multi-head) self-attention sub-layer, and then be further put into a position-wise feed-forward network sub-layer, with each normalized by the layer normalization.

\paragraph{Self-attention sub-layer}
The attention mechanism can be formulated as querying a dictionary with key-value pairs. Formally, $\textrm{Att}(Q, K, V)=\textrm{softmax}(QK^T/\sqrt{d_H}) \cdot V$, where $d_H$ is the dimension of the hidden representations. $Q$, $K$, and $V$ represent query, key, and value. The multi-head variant of attention allows the model to jointly attend to information from different representation sub-spaces, defined as
\begin{align*}
    \textrm{MHA}(Q, K, V) &= [\textrm{head}_1, \ldots, \textrm{head}_A] W^O \\
     \textrm{head}_k &= \textrm{Att}(QW_k^Q, KW_k^K, VW_k^V)  
\end{align*}

\noindent where $[\cdot,\cdot]$ is the concatenation operator, $W_k^Q\in \mathbb{R}^{d_H \times d_K}$, $W_k^K\in \mathbb{R}^{d_H\times d_K}$, $W_k^V\in \mathbb{R}^{d_H\times d_V},$ and $W^O\in \mathbb{R}^{Hd_V \times d_H}$ are projection parameter matrices, $A$ is the number of heads, and $d_K$ and $d_V$ are the dimensions of key and value. 

\paragraph{Position-wise FFN sub-layer}
In addition to the self-attention sub-layer, each Transformer layer also contains a fully connected feed-forward network, which is applied to each position separately and identically. This feed-forward network consists of two linear transformations with an activation function $\sigma$ in between. Specially, given vectors $\mathbf{x}_1, \ldots, \mathbf{x}_n$, a position-wise FFN sub-layer transforms each $\mathbf{x}_i$ as $\text{FFN}(\mathbf{x}_i) = \sigma(\mathbf{x}_iW_1+b_1) W_2 + b_2$, where $W_1, W_2, b_1$ and $b_2$ are parameters.

We should also emphasize that a residual connection \cite{he2016identity} and a layer normalization \cite{ba2016layer} are applied to the output of both MHA or FNN sub-layers. The residual connection plays a key role in learning strict identity mapping (detailed in Section \ref{sec:identity_mapping}), while layer normalization and spectral normalization (detailed in Section \ref{sec:sepctral-normalization}) together ensure regulated magnitude of activation outputs for improved pruning stability.

\subsection{Identity-Inducing Prior for Transformer}
\label{sec:identity_mapping}
% \todo[color=green]{just a thought: should we call this identity-inducing prior? e.g.: ``\textbf{Identity-inducing Prior on  Transformer Layers}"}

The design of residual connection can provide us with a promising way to find identity mappings for the Transformer model. Specifically, residual connection \cite{he2016identity} can be formalized as $\mathcal{H}(\mathbf{x}) = \mathcal{F}(\mathbf{x}) + \mathbf{x}$, where $\mathcal{F}$ could be either $\textrm{MHA}$ or $\textrm{FFN}$ and $\mathcal{H}$ is the sub-layer output.
As illustrated in \citet{he2016deep}, if an identity mapping were optimal, it would be easier to push the residual to zero than to fit an identity mapping by a stack of nonlinear layers.

We leverage $\epsilon$-ResNet \cite{yu2018learning}, a strict identity mapping mechanism that sparsifies the layer output by inducing a specific threshold $\epsilon$ as the \textit{identity prior}.
Specifically, we turn the residual connection $\mathcal{H}(\mathbf{x})$ into $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) + \mathbf{x}$, where 
% \begin{equation*}
% \mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) = 
% \left\{
% \begin{array}{ll}
%     0 &  \textrm{if } |\mathcal{F}(\mathbf{x})_i|<\epsilon, \forall i \in {1, ..., n}\\
%     \mathcal{F}(\mathbf{x}) & \textrm{otherwise}
% \end{array}
% \right.
% \end{equation*}
\begin{equation*}
\mathcal{S}_\epsilon(\mathbf{v}) = 
\left\{
\begin{array}{ll}
    0 &  \textrm{if } |\mathbf{v}_i|<\epsilon, \forall i \in {1, ..., |\mathbf{v}|},\\
    \mathbf{v} & \textrm{otherwise,}
\end{array}
\right.
\end{equation*}

\noindent where $\mathbf{v}_i$ is the $i$-th element of the vector $\mathbf{v}$.
Here a sparsity-promoting function $\mathcal{S}$ is applied to dynamically discard the non-linearity term based on the activations. When all the responses in the non-linear mapping $\mathcal{F}(\mathbf{x})$ is below a threshold $\epsilon$, then $\mathcal{S}(\mathcal{F}(\mathbf{x}))=0$, otherwise, the original mapping $\mathcal{S}(\mathcal{F}(\mathbf{x}))=\mathcal{F}(\mathbf{x})$ was used as the standard residual network.

To implement $\mathcal{S}$, we put an extra binary gate layer $t_\epsilon$ upon $\mathcal{F}(\mathbf{x})$ by stacking additional rectified linear units (ReLU), following \citet{srivastava2015highway}. In particular,
% s = tf.reduce_max(tf.nn.relu(input - epsilon) + tf.nn.relu(-input - epsilon))
%   identity_w = tf.nn.relu(tf.nn.relu(s * (-l) + 1.0) * (-l) + 1.0)
% \begin{align*}
%     \mathcal{T}_1(\mathbf{x}) &= \max\limits_{i \in \{1, ..., n\}}\textrm{ReLU}(|\mathcal{F}(\mathbf{x})_i| - \epsilon), \\
%     \mathcal{T}_2(\mathbf{x}) &= 1 - \textrm{ReLU}(1-\textrm{inf} \cdot \mathcal{T}_1(\mathbf{x})), \\
%     % \mathcal{T}(\mathbf{x}) &= \textrm{ReLU}(1-\textrm{inf} \cdot \mathcal{T}_2(\mathbf{x})), \\
%     \mathcal{S}(\mathcal{F}(\mathbf{x})) &= \mathcal{T}_2(\mathbf{x}) \times \mathcal{F}(\mathbf{x})
% \end{align*}
\begin{equation*}
    t_\epsilon (\mathbf{v}) = 1 - \textrm{ReLU}(1-L \max\limits_{1 \le i \le |\mathbf{v}|}\textrm{ReLU}(|\mathbf{v}_i| - \epsilon))
\end{equation*}

\noindent where $L$ refers to a very large positive constant (e.g., $1e5$ in our experiments). Then, $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{v}))$ has the following form:
\begin{equation*}
    % t = 1 - \textrm{ReLU}(1-\textrm{inf} \cdot \max\limits_{i \in \{1, ..., n\}}\textrm{ReLU}(|\mathcal{F}(\mathbf{x})_i| - \epsilon)), \\
    % \mathcal{T}(\mathbf{x}) &= \textrm{ReLU}(1-\textrm{inf} \cdot \mathcal{T}_2(\mathbf{x})), \\
    \mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) = t_\epsilon (\mathcal{F}(\mathbf{x})) \mathcal{F}(\mathbf{x})
\end{equation*}

Recall that each layer of Transformer consists of two residual blocks, namely, the self-attention sub-layer and the position-wise FFN sub-layer. We apply the $\epsilon$ network directly to the residual block in the FFN sub-layer, i.e., 
% \todo[color=green]{Split this subsection into original attention and multi-head residual variant. Move the former to the preliminary subsection.}
% \todo[color=green]{This S is in fact the F not the S in the eq on line 253. Better rename S.}
\begin{align*}
    \mathcal{H}_\textrm{FFN}(\mathbf{x}) = \mathcal{S}_{\epsilon_\textrm{FFN}}(\textrm{FFN}(\mathbf{x})) + \mathbf{x},
\end{align*}

\noindent When applying it to the attention sub-layer, we employ a modified attention architecture by placing a residual connection to each single attention head, which allows us to prune any subset of attention heads, i.e., \todo{lzi: this is actually not true, there is only one residual connection link to the sum of epsilon(single attention head)}
% every single attention head in each attention sub-layer so that we can prune individual attention head:
\begin{align*}
    \mathcal{H}_\textrm{ATT}(\mathbf{x}) = \sum_{i=1}^A \mathcal{S}_{\epsilon_\textrm{ATT}}(\textrm{head}_i W^O_i) + \mathbf{x}
\end{align*}

\noindent Here, $W^O_i$ is the output weight assign to the $i$-th attention head, i.e., $W^O=[W^O_I, W^O_2, ..., W^O_A]$. If $\mathcal{S}_{\epsilon_\textrm{ATT}}(\textrm{head}_i W^O_i) = 0$, this means that the $i$-th attention head does not contribute to the output of the attention layer and thus could be pruned out.

In our experiment, we set different values to $\epsilon_\textrm{ATT}$ and $\epsilon_\textrm{FFN}$, since the absolute outputs of attention and FFN layers lay in different scalars, as illustrated in Figure \ref{fig:output-distribution}.

% Based on the above definitions, our $\epsilon$-Transformer could be defined as $\mathcal{H}(\mathbf{x}) = \mathcal{S}(\mathcal{F}(\mathbf{x})) + \mathbf{x}$, where $\mathcal{F}(\mathbf{x})$ could be $\textrm{Multi-head}(Q, K, V)$ or $\textrm{FFN}(\mathbf{x})$.

\begin{figure*}[tb]
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/att_output_distibution.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/ffn_output_distibution.pdf}
    \end{minipage}
    \\
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/att_output_distibution_norm=2.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/ffn_output_distibution_norm=2.pdf}
    \end{minipage}
    \caption{Distribution of the max absolute value of the attention/FFN outputs on the Stanford Sentiment Treebank (SST) training set, based on model BERT$_\textrm{BASE}$ (w/o SN) and spectral normalized BERT$_\textrm{BASE}$ (w/ SN). For attention layers, different heads are plotted separately but with the same color in the same layer for clarity.}
    \label{fig:output-distribution}
\end{figure*}

\subsection{Spectral Normalization}
\label{sec:sepctral-normalization}
% motivation of normalizing the weight

% As discussed in Section \ref{sec:identity_mapping}, the sparse-inducing mechanism $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x}))$ takes effect when $|\mathcal{F}(\mathbf{x})_i|<\epsilon$. Clearly, the effectiveness of such a approach relies on a key assumption: within each layer, the statistical distribution of the function norms of the unimportant and the important residual mappings $P(|\mathcal{F}_{\texttt{unimp}}(\mathbf{x})_i|) \, v.s. \, P(|\mathcal{F}_{\texttt{imp}}(\mathbf{x})_i|)$ can be well-separated by $\epsilon$, such that there exists an $\epsilon$ so that the probabilities $P(|\mathcal{F}_{\texttt{unimp}}(\mathbf{x})_i|<\epsilon)$ and $P(|\mathcal{F}_{\texttt{unimp}}(\mathbf{x})_i|>\epsilon)$ are both close to 1. Unfortunately, such separation was not easily observed in the function norm distribution of a standard pre-trained BERT model. For example, in Figure \ref{fig:output-distribution} (Top row), we observe that the function norm distribution for the attention head outputs tend to be densely clustered within the range $[0, 2]$. On the other hand, the norm distribution for the FFN layer outputs varies widely within the range $[0, 1000]$.

In its originally proposal, the sparse-inducing function $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x}))$ were found to work well for randomly initialized neural network, where the initial weight matrix of the nonlinear mappings for all layers were distributed within a consistent range, and thus facilitates a natural separation between the function norms $|\mathcal{F}|$ of the important and unimportant nonlinear mappings in the residual blocks during training \citep{yu2018learning}. This is, however, not the case for the weight distribution for a pre-trainined model like BERT, where the weight distributions between different layers have already diverged during pre-training, likely to due to the specialization of layer functionalities under the masked language modeling (MLM) training \citep{tenney2019bert}. Indeed, in our preliminary experiments, we observed that the proposed identity-inducing prior $\epsilon$ is not effective for a BERT model initialized from a classic pre-training checkpoint. Empirically, as shown in Figure \ref{tab:performance-on-different-norm}, we found the distribution of the function norms $P(|F(\mathbf{x})_i|)$ for the attention layers to be densely clustered within a small range ($(0, 2)$) and with no clear separation between the function norm for the important and unimportant nonlinear residual mappings. On the other hand, the norm distributions for different FFN layers were found to vary wildly, creating challenges for selecting a proper set of $\epsilon$'s in practice.

% In our preliminary experiments, we observed that when applying the defined $\epsilon$-Transformer\todo{another new term? eps-ResNet vs eps-Transformer vs eps network? Maybe add in the previous subsection, we define eps-Transformer as such and such.} to BERT, the distribution of $|\mathcal{F}(\mathbf{x})|$ is of low sparsity\todo{what is sparsity of a distribution? maybe "screwed"?} and the maximum of $|\mathcal{F}(\mathbf{x})|$ for the FFN sub-layer is usually very large, resulting in the difficulty for us to choose a proper set of $\epsilon$.\todo{it's not very clear why these phenomena made it hard to choose eps. shouldn't varied max and distribution across sublayers, layers, and tasks make it hard?}

The above observations motivate us to identify an effective method to stabilize the norm distributions of the BERT model layers. In this work, we consider \textit{Spectral Normalization} (SN), an approach that directly control the Lipschitz norm of a nonlinear mapping $\mathcal{F}$ by regularizing the spectral behavior of its weight matrices \citep{miyato2018spectral}. 

Specifically, for a weight matrix $W$, its spectral norm $\lambda(W)$ is defined as its largest singular value:
\begin{align*}
    \lambda(W) = 
    %\underset{\mathcal{F}_{k-1}}{\textrm{sup}}\sigma(\nabla\mathcal{F}_{k}) = 
    \underset{x\neq0}{\textrm{max}}\frac{||W\mathbf{x}||_2}{||\mathbf{x}||_2}.
\end{align*}
We say a function $\mathcal{F}$ is $L$-Lipschitz if $|\mathcal{F}(x_1)-\mathcal{F}(x_2)|/||x_1 - x_2|| \leq L$, for all $x_1$, $x_2$, and we call the smallest possible $L$ the Lipschitz norm of $\mathcal{F}$, denoted as $|\mathcal{F}|_{Lip}$. 
%In other words, small changes in the input of the function causes corresponding small changes in the magnitude of its gradients. From its definition, the Lipschitz constant of a given layer $k$ of a neural network, whose activations are given by 
Consequently, for a neural network mapping $\mathcal{F}(\mathbf{x}) = \sigma(W\mathbf{x} + b)$ with an contractive activation function $\sigma$,
%\todo{unparsable sentence}
%Similar to other weight normalization methods, spectral normalization normalizes the weight $W$ by the spectral norm (or $L_2$ matric norm), denoted as $\sigma(W)$\todo{sigma is redefined}.
%\noindent which is essentially the largest singular value of the matrix $W$. In our case, spectral normalization guarantees the norm of the function $\mathcal{F}(\mathbf{x})$ resides in a finite region upper bounded by
its Lipschitz norm is upper-bounded by $\lambda(W)$ \citep{miyato2018spectral}:
\begin{equation*}
    |\mathcal{F}|_{Lip} = |\sigma(W \mathbf{x} + b)|_{Lip} \leq |W \mathbf{x} + b|_{Lip} \leq \lambda(W).
\end{equation*}
For BERT models, since the layer input $\mathbf{x}$ follows a  distribution of zero mean and unit variance due to layer normalization \cite{ba2016layer}, a nonlinear mapping's $L_1$ norm $|\mathcal{F}|$ is roughly proportional to its Lipschitz norm $|\mathcal{F}|_{Lip}$, which is controlled by $\lambda(W)$.

Therefore, we are able to have a better control of the maximum of $|\mathcal{F}(\mathbf{x})|$ for identifying a good $\epsilon$. Furthermore, the regularization is achieved by that the layer weights are simply divided by their corresponding spectral norm in SN, i.e. $\hat{W} = W / \hat{\lambda}(W)$, adding no additional trainable  parameter to the original model.

We applied SN to both pre-training and fine-tuning of the BERT model, and on the weights in both the attention and the FFN layers. As shown in Table \ref{tab:performance-on-different-norm}, adding SN to a BERT$_\textrm{BASE}$ model resulted in improved pre-training performance and competitive fine-tuning performance when compared to the original BERT$_\textrm{BASE}$ without SN. To illustrate the effect of SN on the function norms of the BERT model, we plot $|\mathcal{F}(\mathbf{x})|$ for the training set of the Stanford Sentiment Treebank in Figure \ref{fig:output-distribution}. As shown, after SN, the norm distribution $P(|\mathcal{F}_k(\mathbf{x})|)$ between the important and the unimportant nonlinear mappings shows a better separation (Figure \ref{fig:output-distribution}, bottom left), the norms distribution for the FFN layers are now stabilized within a much smaller range (Figure \ref{fig:output-distribution}, bottom right). More examples could be found in the supplementary materials.
%\textbf{Strict weight normalization can sacrifice the expressive power of the network. This could addressed by using less strict Lipschitz constraint $\sigma(W)$, as shown in Table \ref{tab:performance-on-different-norm}.}
% \todo[color=white]{\jzl{this discussion seem to contradict with the statement in the previous paragraph. It might be good to put this discussion to a less prominent place. and mention that strict weight normalization can harm the expressive power of the network due to the existence of the non-gradient-norm preserving activation function, as well as the other regularization mechanisms in the model which scales down the Lipschitz constant in unexpected ways. (you can cite and check out first paragraph of this paper: https://arxiv.org/pdf/1811.05381.pdf)}}
% As excessive normalization can do harm to the model's prediction performance, we found that relatively loosing the target Lipschitz constraint $\sigma(W)$ to some value larger than 1 could have rather negligible or even positive impact on the training process compared to the standard Transformer, as shown in Table \ref{tab:performance-on-different-norm}.

\begin{table}[tb]
    \centering\scalebox{0.8}{
    \begin{tabular}{lcccccc}
    \hline
        \textbf{SN}                  & \textbf{MLM} & \textbf{SST-2} & \textbf{QQP} & \textbf{MRPC} & \textbf{QNLI} & \textbf{MNLI}\\\hline
        w/o                & 71.93       & 92.7        & 90.6        & 90.9         & 91.6         & 84.7           \\
        % BERT$_\textrm{BASE}$ ($\sigma(W)=1$) & 70.72       & 90.4        & 89.0        & 89.2         & 89.0         & 80.6           \\
        % BERT$_\textrm{BASE}$ ($\sigma(W)=2$) & 73.43       & 91.3        & 90.1        & 90.3         & 91.5         & 84.0           \\
        w/ & 74.16       & 91.9        & 90.1        & 90.8         & 91.6         & 85.1           \\
    \hline
    \end{tabular}}
    \caption{Evaluate the performance of BERT$_\textrm{BASE}$ (w/o SN) and the spectral normalized BERT$_\textrm{BASE}$ (w/ SN, using $\lambda(W)=5$), respectively masked language modeling accuracy on pre-training data and accuracy of fine-tuning on 5 natural language understanding tasks (details could be found in Section \ref{sec:datasets}).
    }
    \label{tab:performance-on-different-norm}
\end{table}


% \todo{add an eq between eps and sigma}
% \todo{How to explain that spectral normalization could improve the sparsity of the distribution}
% \todo[color=green ]{jzl: Should we show $\sigma(W)=5$ results instead? Or just change image title to "with spectral regularization"}

% \subsection{Distillation Objective}

% \paragraph{Traditional Distillation} 
% Basically, for training set $\mathcal{D} = {(x^1, y^1), ..., (x^i, y^i))}$, let the output of student model with parameters $\theta$ on the input $x$ be $f(x, \theta)$, and the corresponding output of a well-trained teacher model with parameters $\theta'$ be $f(x, \theta')$. The model distillation trains $\theta$ to minimize the loss on the training set:

% \begin{equation*}
%     \mathcal{L}(\theta)=\sum_{x^i, y^i \in \mathcal{D}}\ell(f(x^i, \theta'), f(x^i, \theta))
% \end{equation*}

% where for classification tasks $\ell$ is the cross entropy loss.

% Several works has proven that we can actually set up the teacher and student have the same neural architecture and model size, but surprisingly the student is able to surpass the teacher's accuracy, which is called Born-Again \cite{furlanello2018born, clark2019bam}. This could be explained by that, distillation is effective because the teacher's output distribution over classes provides more training signal than simple one-hot labels. Given that fact, we start from the student $\epsilon$-Transformer model with the same size as the teacher standard Transformer model. As learning the identity mapping within residual block of the attention and feed forward network, the student will automatically discard the redundant layers.

% \paragraph{Teacher Annealing} In knowledge distillation, the student is trained to imitate the teacher. This raises the concern that the student may be limited bu the teacher's performance and not be able to substantially outperform the teacher. To address this, we use \textit{teacher annealing} proposed by \cite{clark2019bam}, which mixes the teacher prediction with the gold label during training, so the loss function becomes

% \begin{equation*}
%     \mathcal{L}(\theta)=\sum_{x^i, y^i \in \mathcal{D}}\ell(\lambda f(x^i, \theta') + (1-\lambda)y^i , f(x^i, \theta))
% \end{equation*}

% where $\lambda$ refers to how much weight to put on distill targets compared to gold-standard labels.
\begin{figure*}[tb]
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/sst.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/qqp.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/mrpc.pdf}
    \end{minipage}%
    \\
    \begin{minipage}[t]{0.5\textwidth}
        \includegraphics[width=5.5cm, right]{images/performance/qnli.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \includegraphics[width=5.5cm, left]{images/performance/mnli.pdf}
    \end{minipage}
\caption{Evolution of performance when separately pruning attention heads (ATT) and FFN layers (FFN), and joint pruning ATT and FFN (Joint) on 5 GLUE dev sets. * means applying spectral normalization. The percentage pruned (x-axis) is calculated based on the parameters of attention and FFN sub-layers as the full set (excluding embedding, pooler and classifier layers).}
\label{fig:results}
\end{figure*}

\subsection{Iterative Pruning}
The choice of $\epsilon_\textrm{ATT}$ and $\epsilon_\textrm{FFN}$ can be regulated by some prior distribution and optimized during training. We use a simple pruning method that greedily and iteratively prunes away attention heads and FFN layers, which can avoid impractical combinatorial search given the number of attention heads and the time it takes to evaluate each model. The method employs a three-step process: 

(1) Evaluate the output distribution at each iteration to give a heuristics for the selection of $\epsilon$. As $\epsilon$ satisfies a nice monotonicity property --- larger value leads to higher compression, we could start from a relatively low $\epsilon$ and gradually increase it at each iteration. \todo{there should be a problem, since we try to restrict the magnitude but turns out choose $\epsilon$ based on empirical distribution}

(2) Top-down training: train the full-size model with the selected $\epsilon$. Prune the low-weight connections by removing the weights below a threshold. When a residual block produces negligible response, the $\epsilon$ function will start producing $0$ outputs. As a result, the weights in this block will stop contributing to the cross-entropy term. Consequently, the gradients will only based on the regularization term and lead to weight collapse.% It is noted that spectral normalization will help the weight go to zeros more quickly since the largest singular value of the weight has been restricted.

(3) Retrain the compressed model to learn the final weight for the remaining sparse connections. This is critical --- if the pruned network is used without retraining, accuracy is significantly impacted. Also, during retraining, it is better to retain the weights from the initial training phase for the connections that survived pruning than it is to re-initialize them \cite{han2015learning}.
% \todo{Should this subsection be moved to the method section above? +1 to move to method section nhua. Besides "than it is to re-initialize them"?}

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/old/04.experiments.tex <==
\begin{table*}[tb]
    \centering
    \scalebox{0.7}{
    \begin{tabular}{lrccccc}
    \hline
        \textbf{Model}                            & \textbf{FLOPS} & \textbf{ SST-2$_{acc}$} & \textbf{QQP$_{acc}$} & \textbf{MRPC$_{F_1}$} & \textbf{QNLI$_{acc}$} & \textbf{MNLI-mm$_{acc}$}\\\hline
        BERT$_\textrm{BASE}$                      & 22.5B          & \ \ -0.0\%/92.7        & \ \ -0.0\%/90.6       & \ \ -0.0\%/90.9        & \ \ -0.0\%/91.6        & \ \ -0.0\%/84.7 \\
        TinyBERT$_6$ w/o DA \cite{jiao2019tinybert} & 1.2B         & -                      & -                     & -50.0\%/86.0           & -                      & \textbf{-50.0\%/84.4}\\
        DistillBERT$_6$ \cite{sanh2019distilbert} & 11.3B          & -50.0\%/91.3           & -50.0\%/88.5          & -50.0\%/87.5           & -50.0\%/89.2           & -50.0\%/82.2 \\
        BERT-PKD$_6$ \cite{sun2019patient}        & 11.3B          & -50.0\%/91.5           & \textbf{-50.0\%/88.9}          & -50.0\%/86.2           & -50.0\%/89.0           & -50.0\%/81.0 \\
        BERT-PKD$_3$ \cite{sun2019patient}        & 7.6B           & -75.0\%/87.5           & -75.0\%/87.8          & -75.0\%/80.7           & -75.0\%/84.7           & -75.0\%/76.3 \\
        \hline
        % MobileBERT \cite{sun2020mobilebert} *, $\dagger$   & 76.8\%/91.7           & 76.8\%/88.3          & 76.8\%/87.5           & 76.8\%/91.5           & 76.8\%/83.4 \\
        % RPP-BERT$_\textrm{LARGE}$ \cite{guo2019reweighted}& -64.1\%/92.4           & -64.1\%/89.2          & -64.1\%/81.9           & -64.1\%/88.0           & -64.1\%/81.8 \\\hline
        % $\epsilon$-BERT                       & -30.0\%/91.3                 & -38.7\%/89.5                & -39.7\%/89.9                 & -26.1\%/90.8                 & -32.3\%/83.5\\
        FLOP \cite{wang2019structured}           & 15B             & -35.0\%/92.1           & -                     & -35.0\%/88.6           & -35.0\%/89.0           & -           \\
        MvP \cite{sanh2020movement} $\dagger$    & N/A             & -                      & -97.0\%/89.2          & -                      & -                      & -97.0\%/79.7\\\hline\hline
        $\epsilon$-BERT (ours, w/ SN)          & 13.2 - 14.5B    & \textbf{-50.0\%/91.8}           & \textbf{-50.0\%/88.9}         & \textbf{-50.0\%/88.1}           & \textbf{-50.0\%/89.5}           & -50.0\%/82.8\\
        $\epsilon$-BERT (ours, w/ SN)          & 8.3 - 9.1B      & -75.0\%/88.4           & -75.0\%/87.8          & -75.0\%/81.2           & -75.0\%/84.6           & -75.0\%/78.3\\\hline
        $\epsilon$-BERT (ours, w/o SN)                          & 16.8 - 18.2B    & -30.0\%/91.3           & -38.7\%/89.5          & -39.7\%/89.9           & -26.1\%/90.8           & -32.3\%/83.5\\
        % $\epsilon$-BERT ($\sigma(W)=2$)        &                 & -45.3\%/91.3           & -38.6\%/89.7          & -53.3\%/89.8           & -26.7\%/90.5           & -31.4\%/83.6\\
        $\epsilon$-BERT (ours, w/ SN)          & 13.4 - 16.1B    & -56.7\%/91.7           & -40.7\%/89.7          & -46.7\%/89.9           & -36.0\%/90.7           & -39.3\%/83.9\\
        \hline
    \end{tabular}}
    \caption{The compression results including model efficiency (percentage of reduced parameters) and performance from the GLUE dev results, and the MNLI result is evaluate for mismatched-accuracy (MNLI-mm). BERT$_\textrm{BASE}$ indicates the results of the fine-tuned BERT$_\textrm{BASE}$ in our implementation. The number of model parameters includes the attention and FFN sub-layers but excludes the embedding, pooler and classifier layers. The bold numbers indicate the best performance for keeping 50\% of the parameters respectively. $\dagger$ means unstructured pruning, which could not speed up the inference in practice.}% The RPP-BERT was trained based on BERT$_\textrm{LARGE}$, which means it can be unfair to make a direct comparison.} %* means part of the pruned parameters comes from the embedding layers, and $\dagger$ means the compression is task-agnostic.}
    \label{tab:best-architecture}
\end{table*}

\todo{lzi: is the last two lines of the table necessary? since it could actually be read from Figure 3.}
\section{Experiments}
% \todo[color=green]{Figure 1 and table 1 are not referenced in the content.}
% \todo[color=green]{Increase fonts for all figures.}

\subsection{Experimental Settings}
In the experiments, we apply the same architecture and the base settings from the original BERT$_\textrm{BASE}$ \cite{devlin2018bert}, and fine-tune each task independently. More details could be found in supplementary materials.
\todo{weight based pruning baselines?}

% The key hyperparameters are the thresholds $\epsilon_{ATT}$ and $\epsilon_{FFN}$, where we apply an iterative pruning as discussed in the next subsection.

\subsection{Datasets}
\label{sec:datasets}
For pre-training, we use the same data as BERT, which consists of 3.3 Billion tokens from Wikipedia and BooksCorpus \citep{zhu2015aligning}. 
For fine-tuning tasks, we conduct experiments on the subset of the General Language Understanding Evaluation (GLUE) Benchmark \citep{wang2018glue}, classified into three categories: (1) sentiment analysis: Stanford Sentiment Treebank (SST, \cite{socher2013recursive}); (2) paraphrasing: Quora Question Pairs (QQP, \cite{chen2018quora}), Microsoft Research Paraphrase Corpus (MRPC, \cite{dolan2005automatically}); (3) natural language inference: Question Natural Language Inference (QNLI, \cite{chen2018quora}), Multi-genre Natural Language Inference (MNLI, \cite{williams2017broad}). The reason for choosing this subset is that we found the variance in performance for those tasks lower than the other GLUE tasks. Further details about those tasks could be found in supplementary materials.
% \todo[color=green]{Reasons for the subset use like Dan said.}

\subsection{Results}
We compare the pruning results on non-normalized and normalized BERT models on the 5 GLUE tasks, as shown in Figure \ref{fig:results}, which includes separate pruning for attention heads and FFN sub-layers and joint pruning for both sub-modules. The results demonstrate the advantage of using spectral normalization.\textbf{ To put it all together, in Table \ref{tab:best-architecture}, we further show the simplest architecture we could get when allowed at most 1\% in terms of  performance degradation. This also means that further slight pruning will have noticeable impact on the final results. }
%where we first trained the pruning of attention heads and FFN layers separately to get the full evolution of the performance during the training process.

% Finally, to put it all together, we dynamically train the pruning of both attention heads and FFN sub-layers. The final $\epsilon$-BERT allows us to choose the simplest architecture corresponding to any negligible results, and in Table \ref{tab:best-architecture}, we further show the simplest architecture we could get when allowed at most 1\% in terms of  performance degradation. This also means that further slight pruning will have noticeable impact on the final results. 

We also list other compression methods in the table for comparison while most of them are of knowledge distillation and have a pre-defined fixed size of the compressed model.
Our methods provide the flexibility to choose the best architecture and take the advantage of finding the inflection point during pruning, while compared with other pruning methods we could practically speed up the inference time since we use a structured pruning.
\footnote{TinyBERT \cite{jiao2019tinybert} utilizes data augmentation (DA) to improve the distillation results, which makes it unfair to have a direct comparison, so here we only listed their results without DA. As for the unstructured pruning in MvP \cite{sanh2020movement}, current hardware does not support optimized inference for the sparse model so it is actually hard to put it in practice. We do not list the results in \citet{guo2019reweighted, gordon2020compressing} since they show the results in scatter plots instead of the exact numbers, and similarly they are of unstructured pruning.}%i.e, though some models save more parameters, their results are far below the original BERT, without noticing that: (1) actually slightly adding more parameters could keep almost the same performance, (2) sometimes compressing further still does no harm, and (3) different tasks need different model size. Furthermore, unlike other models, $\epsilon$-BERT does not need to transfer the knowledge of each layer from the teacher model or doing data augmentation to provide more task-specific data.

==> Pruning Redundant Mappings in Transformer Models via Spectral-normalized Identity Prior/sections/old/05.ablation_study.tex <==
\begin{figure*}[tb]
    \centering
    \begin{tabular}{p{0.005\textwidth}p{0.28\textwidth}p{0.28\textwidth}p{0.28\textwidth}}
            & \multicolumn{1}{c}{\ \ \ \ \ SST}   & \multicolumn{1}{c}{\ \ \ \ \ MRPC} &\multicolumn{1}{c}{\ \ \ \ \ MNLI} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 16.67\%} &  \includegraphics[width=0.3\textwidth]{images/ablation/sst/sst_iter1.pdf}    & \includegraphics[width=0.3\textwidth]{images/ablation/mrpc/mrpc_iter1.pdf} & \includegraphics[width=0.3\textwidth]{images/ablation/mnli/mnli_iter1.pdf} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 33.33\%} &  \includegraphics[width=0.3\textwidth]{images/ablation/sst/sst_iter2.pdf}    & \includegraphics[width=0.3\textwidth]{images/ablation/mrpc/mrpc_iter2.pdf} & \includegraphics[width=0.3\textwidth]{images/ablation/mnli/mnli_iter2.pdf} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 50.00\%} &  \includegraphics[width=0.3\textwidth]{images/ablation/sst/sst_iter3.pdf}    & \includegraphics[width=0.3\textwidth]{images/ablation/mrpc/mrpc_iter3.pdf} & \includegraphics[width=0.3\textwidth]{images/ablation/mnli/mnli_iter3.pdf}
    \end{tabular}
    \caption{Faded map of attention heads and FFN layers during pruning on task SST-2, MRPC and MNLI dev sets. Color white indicates that this attention head or FFN layer has been entirely pruned out. The left column shows the percentage pruned, and \texttt{mean} is the mean of attention heads of each layers.}
    \label{fig:heatmap}
\end{figure*}

\begin{figure}[tb]
    \centering
    \includegraphics[width=6cm]{images/ablation/ablation.pdf}
    \caption{Evolution of accuracy on the dev set of SST-2 for (1) pruning the whole attention layers (HA); (2) pruning single attention heads (MHA); (3) layer pruning means pruning the whole layer (Layer pruning) and (4) pruning the attention and FFN sub-layers separately (Split pruning).}
    \label{fig:abaltion}
\end{figure}

\section{Ablation Study}
In this section, we investigate the contribution of: (1) single attention head pruning, and (2) split pruning for attention heads and FFN sub-layers.

\paragraph{Single Head Attention Pruning}

Multi-head self-attention is a key component of Transformer, where each attention head potentially focusing on different parts of the inputs. The analysis of multi-head attention and its importance is challenging. Previous analysis of multi-head attention considered the average of attention weights over all heads at given position or focused only on the maximum attention weights \cite{voita2018context, tang2018analysis}, or explicitly takes into account the varying importance of different heads \cite{voita2019analyzing}. Moreover, \citet{michel2019sixteen} has proved that a large percentage of attention heads can be removed at test time without significantly impacting performance, but they mainly discussed the case on machine translation and NLI tasks, and it is still unknown whether attention heads play consistent and interpretable roles when trained on different downstream tasks.

To probe this question, we pick one task from the sentiment analysis, paraphrasing and natural language inference respectively, plot the pruned attention heads during training and show the dynamic process in Figure \ref{fig:heatmap}, where we can find that though for different tasks, the distribution of important attention heads are similar, as reflected in the mean of each attention layer, but the exact pruned attention heads are actually different. This also indicates that splitting the pruning for attention heads could have more flexibility for the model to find an optimal architecture.

\paragraph{Separate Pruning for Attention and FFN}
% To allow the different attention heads to interact with each other, the Transformer model applies a non-linear feed-forward network over the multi-head attention's output at each layer \cite{vaswani2017attention}. 
Decoupling and then individually studying the self-attention and the FFN sub-layers is important for understanding the progressive improvement they provide.
As can be observed from Figure \ref{fig:results}, for most of the tasks, the negative effect brought by pruning FFN layers are way more significant than attention layers, indicating that the compression technique for the Transformer model is usually highly effective on the attention layers \cite{voita2018context, michel2019sixteen}, but may be less successful on the fully connected layers \cite{ganesh2020compressing}. In Figure \ref{fig:heatmap}, similar to attention heads, we further plot the faded map of FFN layers, and find that, certain FFN sub-layers might be more amenable to compression, even if the corresponding self-attention sub-unit is not. For example, in all the tasks, the FFN layer near the ends of input or output are more likely to be pruned, while this is not the case for the corresponding self-attention layers.

Finally, to valid the advantage of the single head attention pruning and split pruning for attention/FFN, we further show the evolution of performance for single head attention pruning (HA), multi-head attention pruning (MHA), separate attention/FFN pruning, and whole layer pruning respectively in Figure \ref{fig:abaltion}.

% The compression technique for the Transformer model is usually highly effective on the attention layers \cite{voita2018context, michel2019sixteen}, but may be less successful on the fully connected layers, while clearly the latter part consuming the most memory and executing the highest number of Floating Point Operations Per Second (FLOPS).



==> sections/old/01.introduction.tex <==
\section{Introduction}


% \todo[color=green]{Dan: all the captions of the Figure and Table should stand alone without further reference on the text}
\begin{figure}[t]
    \centering
    \includegraphics[width=6.5cm]{images/others/mnli_prune.pdf}
    \caption{Comparison of selected knowledge distillation (KD) methods (DistilBERT \cite{sanh2019distilbert} and BERT-PKD \cite{sun2019patient}) and iterative pruning (IP) methods (Iterative Pruning \cite{guo2019reweighted} and our proposed method) in terms of accuracy at various compression rate using MNLI test set. KD methods require re-distillation from the teacher to get each single data point, whereas IP methods can produce continuous curves at once.}
    \label{fig:example}
    \vspace{-10pt}
\end{figure}

Natural Language Processing (NLP) has recently achieved great success by using the Transformer-based pre-trained models \cite{radford2019language, devlin2018bert, yang2019xlnet, clark2020electra}. However, these models often consume considerable storage, memory bandwidth, and computational resource. To reduce the model size and increase the inference throughput, compression techniques such as knowledge distillation \cite{sanh2019distilbert, sun2019patient, tang2019distilling, jiao2019tinybert, sun2020mobilebert} and weight pruning \cite{guo2019reweighted, wang2019structured, gordon2020compressing, sanh2020movement} have recently been developed. Knowledge distillation methods require a predefined fixed architecture (referred to as the \emph{student}) as a \emph{priori}, which often has to be identified by a tedious sequence process of trial-and-error. In comparison, iterative pruning methods gradually prune the redundant model weights or layers from the full-size model, and provides the full picture of the trade-off between the task performance and the model size with a single training process, as illustrated in Figure \ref{fig:example}.
% For example, in Figure \ref{fig:example} we show the performance on BERT fine-tuning task of iterative weight pruning \cite{guo2019reweighted}
% \todo[color=green]{This is not our method? And why the citation here is different from the one in the figure caption?}
% and two knowledge distillation methods \cite{sanh2019distilbert, sun2019patient}, where we can see that each performance point of knowledge distillation requires a trial of training, while pruning could provide the full image of the trade-off with a single training process, thus has more flexibility to find an optimal architecture.
%For instance, BERT \citep{devlin2018bert}, a widely-adopted pre-trained language representation model, has significantly improved the state-of-the-art across 11 different NLP tasks. However, these models consume considerable storage, memory bandwidth, and computational resource.

%It sometimes can only realistically be trained in large industrial research laboratories and such models trained with model parallelism cannot even be fine-tuned on a single GPU as their memory requirements demand a multi-accelerator hardware setup even for a single training step \citep{kitaev2020reformer}.

% To fulfill the deployment in real-time applications, many recent studies have been focused on making those giant models more efficient. Existing solutions include model parallelization \cite{} and model compression \cite{}. The former addresses the memory limitation problems, but not the communication overhead, while the latter aims to designing a lite version of the original architecture that has significantly fewer parameters.



% \todo[color=green]{Dan: perhaps add a figure show the difference of kd and wp, like Figure \ref{fig:abaltion}?}

% The former approach is ``bottom-up'', in the sense that it specifies a fixed architecture for the final compressed model as the priori. Based on this scenario, it is often loosely guided by a tedious sequence process of trial-and-error based decisions. Unlike knowledge distillation, weight pruning is ``top-down'', in the sense that it starts from the full size and prunes the redundancy in the weights/layers of the model.

Although iterative pruning methods make it easy to determine the most compact architecture given a required task performance, many focus on using sparsity-promoting regularizers to promote individual weight which can be arbitrary and usually irregular \cite{guo2019reweighted, sanh2020movement}. It actually cannot achieve superior runtime performance or even adversely impact practical acceleration in hardware platforms when compared with directly reducing numerical component modules \cite{wen2016learning}. On the other hand, previous works have questioned the importance of different component modules in the Transformer model and found that different components learn different levels of knowledge. For a specific downstream task, there are unimportant sub-modules focusing on knowledge not preferred by the task \cite{tenney2019bert, liu2019linguistic, jawahar2019does, kovaleva2019revealing}, i.e., those modules only provide relatively identical mappings that are not contributing to the final output. Therefore, we believe that these task-specific unimportant identity mappings could be identified and discarded by leveraging some \emph{identity priors}.

% \todo[color=green]{Can revive the pruning. Focus on the limitation of pruning.}
% \todo[color=green]{Briefly mention both distillation and pruning methods and explain them in the top-down/bottom-up way.}
% \todo[color=green]{also can mention that pruning is often regarded as a simpler compression method than distillation}

% \textbf{Discuss the unstructured and structured pruning: }For weight pruning, most of the previous works consider different sparsity-promoting regularization schemes for individual weights \cite{guo2019reweighted, sanh2020movement}. However, it often produces non-structured random connectivity and thus, irregular memory access that adversely impacts practical acceleration in hardware platforms \cite{wen2016learning}. %Furthermore, as illustrated in \citet{Brunner2020On}, there can be infinitely many different attention weights that yield the same output, thus the model redundancies are actually across different layers instead of only within each individual weights.

In this paper, we propose a \emph{structured} pruning method to prune higher-level mappings as a whole, e.g. a single attention head, an attention module, a feed-forward subnetwork, etc. in a Transformer-based model.
Specifically, we take the advantage of the residual blocks ($\mathcal{F}(x) + x$) of a Transformer layer and compress them to \emph{strict identity mappings} \cite{yu2018learning} by identifying the residual blocks whose nonlinearity activations ($\mathcal{F}(x)$) mostly fall below a threshold $\epsilon$.
% Specifically, the model will automatically discard redundant layers by learning \textit{strict identity mapping} \cite{yu2018learning} of the residual block, whose basic idea is that a ``useful'' layer should have magnitude above a certain threshold, so that we could discard those unimportant layers by ruling out those whose magnitudes are under the threshold. \textbf{In this way, the model could be more sparse at the level of layer mapping instead of individual weight.} 
% Several recent works have been focusing on large-scale pre-training models, among which a most widely-used technology is knowledge distillation \citep{hinton2015distilling}, where a compact model (the \textit{student}) is trained to reproduce the behavior of a larger model (the \textit{teacher}) or an ensemble of models \cite{sanh2019distilbert, sun2019patient, sun2020mobilebert, jiao2019tinybert}.
% While knowledge distillation has been proven to be a promising way to compress a large model into a small model, in the basic scenario, it requires the priori to pre-define the student's architecture, which is a tedious sequential process, often loosely guided by a sequence of trial-and-error based decisions to identify a smaller network architecture. This motivates us to develop a more principled approach to identifying optimal student architectures. 
% On the other hand, a model with smaller capacity can also be obtained by other model compression techniques such as sparsification, quantization, pruning and regularization, or even with their combinations, e.g., \citet{mishra2018apprentice} and \citet{polino2018model} are some works that combine knowledge distillation with quantization; \citet{theis2018faster} and \citet{ashok2018nn} combine distillation with pruning.
% In supervised learning, a classification model is generally trained to predict an instance class by maximizing the estimated probability of gold labels. A standard training objective thus involves minimizing the cross-entropy between the model's predicted distribution and the one-hot empirical distribution of training labels. A model performing well on the training set will predict an output distribution with high probability on the correct class and with near-zero probabilities on other classes. But some of these ``near-zero'' probabilities are larger than others and reflect, in part, the generalization capabilities of the model and how well it will perform on the test set. For example, the language representation model BERT \cite{devlin2018bert}'s predictions for a masked token in ``\texttt{I think this is the beginning of a beautiful [MASK]}'' comprise two high probability tokens (\textit{day} and \textit{life}) and a long tail of valid predictions (\textit{future, story, world}). 
% \todo[color=green]{lzi: the following three paragraphs seem to lose coherence}
However, the weight of the Transformer model could be still under-regularized when using simple $L_1$ or $L_2$ based regularizers, making the magnitude of the activation functions prone to be noisy even after layer normalization \cite{ba2016layer}.
% However, the problem of applying this approach to models like BERT is that, during task fine-tuning the weights are starting from pre-training, and the magnitude of the activation function is under-regularized, making the sparsity learning of fine-tuning less than guaranteed.
To address this issue, we further propose to leverage \emph{spectral normalization} \cite{miyato2018spectral} to restrict the largest singular value of the weight metrics in order to stabilize the magnitude (norm) of the activation functions.

While the proposed method could be applied to any Transformer-based network that has residual blocks, we use BERT \cite{devlin2018bert} as a case study in this paper.
We compare the performance of various compression methods across multiple tasks in the GLUE benchmark \citep{wang2018glue} and show that our proposed method improves the performance over the state-of-the-art by $+0.5 \sim 1.0\%$ on average at 50\% compression ratio.
% in paraphrsing, natural language inference and sentiment classification, where 
% we provide a clear task-dependent comparison on model complexity and their corresponding prediction performance, and achieve comparable results on some specific model sizes.
We also validate that by using spectral normalization, we could obtain more sparse and regulated layer mappings during BERT model pre-training, and compress to a model that can outperform the one pruned from the BERT model only with the ReLU activation function.
In the ablation study, we further compare the remaining model components across the tasks at the same compression ratio, and show that the remaining components are similar but not exactly identical.

% Another concern for the compression methodology is that whether we should have a task-agnostic or task-independent compressed model. As illustrated in previous work \cite{tenney2019bert, liu2019linguistic,jawahar2019does}, different layers of the model learn different levels of knowledge from the training data, while only certain part of the learned knowledge is needed for a specific downstream task. Therefore, different tasks theoretically should correspond to different model sizes, but what is the optimal structure combination and is this task-general still remain non-obvious. From an in-depth analysis of the pruning of separate model components, i.e., the attention and FFN sub-layers, we demonstrate that the redundancy components of the model are similar across different tasks but are not extremely identical. \todo{Motivate task-specific compression after introduction of model compression.}

% task-specific trade-off between computational complexity and prediction performance via structured sparse pruning on the attention heads and feed-forward functions in the Transformer model iteratively. 
% \todo{lzi: keyword: pruning - structured - mappings}
Our contributions are three-fold: First, we propose a structured pruning method applicable to mappings instead of individual weights,
which can iteratively identify an ideal architecture while practically achieve inference speedup.
Also, we novelly use spectural normalizated identity prior for BERT to obtain well-regularized weights and sparse layer mappings. 
Finally, we empirically show that on different downstream tasks, different model components play different critical roles, suggesting that we need to perform task-specific pruning to obtain different architectures.
% \todo[color=green]{Should this fact be observed by with some probing work also?}

==> sections/old/02.related_work.tex <==
\section{Related Work}
\paragraph{Pre-trained Language Model Compression}
The major existing efforts to compress pre-trained language models such as BERT can be generally categorized into two lines: knowledge distillation \cite{ba2014deep, hinton2015distilling} and pruning \citep{iandola2016squeezenet, veit2017convolutional}. Other approaches include weight sharing \cite{liu2019roberta}, quantization \cite{zafrir2019q8bert, shen2019q} and neural architecture search \cite{chen2020adabert}, but are much more complicated and not within the discussion of this paper. \todo{lzi: might need to have a reason for skipping the discussion for other approaches?}

The knowledge distillation approach enables the transfer of knowledge from a large \textit{teacher} model to a smaller \textit{student} model, \textbf{which is improved in the process}. A line of works has been dealing with the knowledge distillation for the large-scaled Transformer-based model BERT, e.g., DistillBERT \cite{sanh2019distilbert}, BERT-PKD \cite{sun2019patient}, Distilled BiLSTM \cite{tang2019distilling}, TinyBERT \cite{jiao2019tinybert}, MobileBERT \cite{sun2020mobilebert}, etc.
However, state-of-the-art knowledge distillation methods share a common feature: they require carefully \textit{hand-designed} architectures for the student model, and this process makes it very difficult to explore the full spectrum of trade-offs and find the best affordable one. Furthermore, to choose which intermediate results that the student model can learn from, e.g., the outputs of each layers, the attention maps, are still under discussion.
% \todo{nhua: (it's confusing to me on "optimal", maybe) they require carefully \textit{hand-designed} architectures for the student model, and it's  difficult to explore the full spectrum of tradeoffs and find the best affordable. (Note that I doubt think this argument is strong enough while I can't do better)}

For pruning-based methods, the model is progressively removed, and therefore narrows the range of least important weight or connections. 
For language representation models, many of the existing work focus on unstructured or structured pruning of individual weights matrices. For example, \citet{guo2019reweighted} integrates reweighted $\textit{l}_1$ minimization with a proximal algorithm to search sparsity patterns in the model; \citet{wang2019structured} proposes a structured pruning approach based on low-rank factorization and augmented Lagrangian $\textit{l}_0$ norm regularization; \citet{gordon2020compressing} uses magnitude weight pruning, which compresses the model by removing weights close to 0; \citet{sanh2020movement} applies deterministic first-order weight pruning method where both weights with low and high values can be pruned. On the other hand, within the context of the transformer model, there also exists work that focuses on pruning a coherent set of sub-modules. The examples include 
\citet{michel2019sixteen} and \citet{voita2019analyzing} that prunes individual attention heads either manually via certain head importance score, or automatically via a relaxed $L_0$ regularization, and also \citet{fan_reducing_2020} that applies random pruning to the entire layers. Our work differs from these approaches in that we consider a principled pruning strategy that allows fine-grained pruning on all transformer modules (i.e., both the attention heads and the feed-forward layers), and we study the benefit of improving the mathematical property of a transformer (i.e. Lipschitz condition) to the effectiveness of pruning.
% \todo[color=white]{\jzl{below statements are a bit strong since there do exist module /  layer-wise pruning approaches. I added few sentences about module-wise/layer-wise approaches above , PTAL. }}
%\textbf{However, these works focus on either unstructured or structured pruning on the individual weight matrices, while none has tried a more structured way to prune at the layer level.} \todo{What is the disadvantage of those works? Why should we try pruning at layer / function / activation level?} \todo{LayerDrop?}
% \todo[color=green]{Is the focus to compare weight based vs activation based?}

% There are many work dealing with the model 
% BERT \cite{devlin2018bert} is a Transformer model pre-trained on large corpora using two training objectives: Masked Language Model (MLM), which helps it learn the context in a sentence, and Next Sentence Prediction (NSP), where it learns the relationship between two sentences. Transformer-based models can be compressed using low-rank approximation, weight sharing, knowledge distillation, quantization, or pruning.

% \paragraph{Language Representation Models} Learning representations of natural language has been shown to be useful for a wide range of NLP tasks and has been widely adopted \cite{mikolov2013distributed, dai2015semi, peters2018deep, devlin2018bert, radford2019language}.
% One of the most significant changes in the last two years is the shift from pre-training word embeddings, whether standard \cite{mikolov2013distributed, pennington2014glove} or contextualized \cite{mccann2017learned, peters2018deep}, to full-network pre-training followed by task-specific fine-tuning \cite{dai2015semi, radford2019language, devlin2018bert}. 

% The most well-known example is BERT \cite{devlin2018bert}, a Transformer model pre-trained on large corpora using two training objectives: Masked Language Model (MLM), which helps it learn the context in a sentence, and Next Sentence Prediction (NSP), where it learns the relationship between two sentences. Other Transformer-based pre-trained models includes GPT-2 \cite{radford2019language}, XLNet \cite{yang2019xlnet}, ELECTRA \cite{clark2020electra}, T5 \cite{raffel2019exploring}, etc.

% However, those most recently Transformer-based models often have over billion parameters, which can be prohibitively costly. This problem is exacerbated when we consider devices with lower capacity, e.g., smartphones, and applications with strict latency constraints, e.g., interactive chatbots or search engine. Therefore, efficient methods for compressing those models are desperately in need.\todo{I would probably discard this subsection. Instead, add a preliminary subsection at the beginning of next section to review BERT architecture.}


% To achieve this goal for the Transformer-based model, many works consider leveraging different sparse-promoting regularization schemes, e.g., $\textit{l}_0$ regularization \cite{voita2019analyzing, wang2019structured}, (reweighted) $\textit{l}_1$ regularization \cite{guo2019reweighted}. 
% A prominent line of work is devoted to compressing large neural networks to accelerate inference. Early pioneering works mainly targeted on convolutional neural networks (CNNs) \citep{lecun1990optimal, han2015deep, li2016pruning, liu2017learning, tang2018flops, chen2018constraint, wu2018training}, while many actually could be applicable to Transformers. Common techniques include (1) quantization, which uses fewer bits to represent the parameters, e.g., \citet{hubara2017quantized}, \citet{zafrir2019q8bert}, and \citet{shen2019q}; (2) pruning, which removes less important parameters, including sparse pruning that focuses on locating the set of least important weights in the model \citep{guo2019reweighted, gordon2020compressing}, and structured pruning that focuses on pruning the architectural components \cite{kovaleva2019revealing, michel2019sixteen, raganato2020fixed}; (3) parameter sharing across similar model units \cite{lan2019albert}.

% Other work tries to apply a differentiable neural architecture search for the original models \cite{chen2020adabert}.

% \paragraph{Strict Identity Mapping}
% In this paper, we introduce strict identity mapping, or residual pruning into the Transformer model, which was originally proposed by \cite{yu2018learning} and used in ResNet \cite{he2016deep}.

%Therefore, towards a more principled approach to network architecture compression, many works have been trying to combine traditional compression with knowledge distillation \cite{mishra2018apprentice, polino2018model, theis2018faster, ashok2018nn}, but very few works deal with the transformer model.


% Typical approaches include (1) sparse decomposition \cite{liu2015sparse}; (2) sparsity regularizer \cite{alvarez2016learning, wen2016learning}, which defines a group sparsity regularizer on the parameters of the network; (3) weight elimination \cite{han2015deep, han2015learning}, which learns the sparsity pattern of network weights by eliminating weight whose absolute value is less than an empirical threshold; (4) strict identity mapping \cite{yu2018learning}.

% \paragraph{Invertible Network} Invertible Network, first introduced in \cite{gomez2017reversible}, could address the issue of memory consumption when training a giant model. As one needs to store the activations in order to calculate gradients using backpropagation, making the network invertible allows us to reconstruct each layer's activations exactly from the next layer's, resulting in freeing the memory of the activations for most layers. Recently, a line of works begin to develop invertible variants \cite{gomez2017reversible, jacobsen2018revnet, behrmann2018invertible, kitaev2020reformer} of widely-used deep learning models such as ResNet \cite{he2016deep} and Transformer \cite{vaswani2017attention}. Typically, enforcing invertibility requires partitioning dimensions or modifying network architectures and negligible performance change need to be pre-guaranteed \cite{gomez2017reversible, jacobsen2018revnet, kitaev2020reformer}. Recently, \cite{behrmann2018invertible} showed that standard ResNet architectures can be made invertible by adding a simple normalization in standard frameworks. We will further introduce this normalization in Section \ref{ref:sepctral-normalization}.


\paragraph{Applications of Spectral Normalization}
%\todo{Add subsection to residual pruning and spectral norm}

Spectral normalization is first proposed for generative adversarial network (GAN)  
as a regularization technique to stabilize the discriminator training \citep{miyato2018spectral}. It was later applied to improve the performance of the other types of generative neural networks \citep{zhao_adversarially_2018, behrmann_invertible_2019}, and was analyzed theoretically in the context of adversarial robustness and generalization \citep{farnia_generalizable_2018}. In this paper, we will explore the benefit of spectral regularization for improving the effectiveness of pruning.

==> sections/old/03.method.tex <==
\section{Method}

% In this section, we will lay the theoretical groundwork for our proposed method.
In this section, we describe in the detail the proposed iterative mapping pruning method.

\subsection{Background: Transformer Layer}
Transformer-based models are usually comprised of a stack of Transformer layers. A Transformer layer takes on a sequence of vectors as input, first passes it through a (multi-head) self-attention sub-layer, followed by a position-wise feed-forward network sub-layer.%\textbf{ It outputs a new sequence of vectors of the same shape.}
% The computation inside a layer is decomposed into two steps: the vector first pass through a (multi-head) self-attention sub-layer, and then be further put into a position-wise feed-forward network sub-layer, with each normalized by the layer normalization.

\paragraph{Self-attention sub-layer}
The attention mechanism can be formulated as querying a dictionary with key-value pairs. Formally, $\textrm{Att}(Q, K, V)=\textrm{softmax}(QK^T/\sqrt{d_H}) \cdot V$, where $d_H$ is the dimension of the hidden representations. $Q$, $K$, and $V$ represent query, key, and value. The multi-head variant of attention allows the model to jointly attend to information from different representation sub-spaces, defined as
\begin{align*}
    \textrm{MHA}(Q, K, V) &= [\textrm{head}_1, \ldots, \textrm{head}_A] W^O \\
     \textrm{head}_k &= \textrm{Att}(QW_k^Q, KW_k^K, VW_k^V)  
\end{align*}

\noindent where $[\cdot,\cdot]$ is the concatenation operator, $W_k^Q\in \mathbb{R}^{d_H \times d_K}$, $W_k^K\in \mathbb{R}^{d_H\times d_K}$, $W_k^V\in \mathbb{R}^{d_H\times d_V},$ and $W^O\in \mathbb{R}^{Hd_V \times d_H}$ are projection parameter matrices, $A$ is the number of heads, and $d_K$ and $d_V$ are the dimensions of key and value. 

\paragraph{Position-wise FFN sub-layer}
In addition to the self-attention sub-layer, each Transformer layer also contains a fully connected feed-forward network, which is applied to each position separately and identically. This feed-forward network consists of two linear transformations with an activation function $\sigma$ in between. Specially, given vectors $\mathbf{x}_1, \ldots, \mathbf{x}_n$, a position-wise FFN sub-layer transforms each $\mathbf{x}_i$ as $\text{FFN}(\mathbf{x}_i) = \sigma(\mathbf{x}_iW_1+b_1) W_2 + b_2$, where $W_1, W_2, b_1$ and $b_2$ are parameters.

We should also emphasize that a residual connection \cite{he2016identity} and a layer normalization \cite{ba2016layer} are applied to the output of both MHA or FNN sub-layers. The residual connection plays a key role in learning strict identity mapping (detailed in Section \ref{sec:identity_mapping}), while layer normalization and spectral normalization (detailed in Section \ref{sec:sepctral-normalization}) together ensure regulated magnitude of activation outputs for improved pruning stability.

\subsection{Identity-Inducing Prior for Transformer}
\label{sec:identity_mapping}
% \todo[color=green]{just a thought: should we call this identity-inducing prior? e.g.: ``\textbf{Identity-inducing Prior on  Transformer Layers}"}

The design of residual connection can provide us with a promising way to find identity mappings for the Transformer model. Specifically, residual connection \cite{he2016identity} can be formalized as $\mathcal{H}(\mathbf{x}) = \mathcal{F}(\mathbf{x}) + \mathbf{x}$, where $\mathcal{F}$ could be either $\textrm{MHA}$ or $\textrm{FFN}$ and $\mathcal{H}$ is the sub-layer output.
As illustrated in \citet{he2016deep}, if an identity mapping were optimal, it would be easier to push the residual to zero than to fit an identity mapping by a stack of nonlinear layers.

We leverage $\epsilon$-ResNet \cite{yu2018learning}, a strict identity mapping mechanism that sparsifies the layer output by inducing a specific threshold $\epsilon$ as the \textit{identity prior}.
Specifically, we turn the residual connection $\mathcal{H}(\mathbf{x})$ into $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) + \mathbf{x}$, where 
% \begin{equation*}
% \mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) = 
% \left\{
% \begin{array}{ll}
%     0 &  \textrm{if } |\mathcal{F}(\mathbf{x})_i|<\epsilon, \forall i \in {1, ..., n}\\
%     \mathcal{F}(\mathbf{x}) & \textrm{otherwise}
% \end{array}
% \right.
% \end{equation*}
\begin{equation*}
\mathcal{S}_\epsilon(\mathbf{v}) = 
\left\{
\begin{array}{ll}
    0 &  \textrm{if } |\mathbf{v}_i|<\epsilon, \forall i \in {1, ..., |\mathbf{v}|},\\
    \mathbf{v} & \textrm{otherwise,}
\end{array}
\right.
\end{equation*}

\noindent where $\mathbf{v}_i$ is the $i$-th element of the vector $\mathbf{v}$.
Here a sparsity-promoting function $\mathcal{S}$ is applied to dynamically discard the non-linearity term based on the activations. When all the responses in the non-linear mapping $\mathcal{F}(\mathbf{x})$ is below a threshold $\epsilon$, then $\mathcal{S}(\mathcal{F}(\mathbf{x}))=0$, otherwise, the original mapping $\mathcal{S}(\mathcal{F}(\mathbf{x}))=\mathcal{F}(\mathbf{x})$ was used as the standard residual network.

To implement $\mathcal{S}$, we put an extra binary gate layer $t_\epsilon$ upon $\mathcal{F}(\mathbf{x})$ by stacking additional rectified linear units (ReLU), following \citet{srivastava2015highway}. In particular,
% s = tf.reduce_max(tf.nn.relu(input - epsilon) + tf.nn.relu(-input - epsilon))
%   identity_w = tf.nn.relu(tf.nn.relu(s * (-l) + 1.0) * (-l) + 1.0)
% \begin{align*}
%     \mathcal{T}_1(\mathbf{x}) &= \max\limits_{i \in \{1, ..., n\}}\textrm{ReLU}(|\mathcal{F}(\mathbf{x})_i| - \epsilon), \\
%     \mathcal{T}_2(\mathbf{x}) &= 1 - \textrm{ReLU}(1-\textrm{inf} \cdot \mathcal{T}_1(\mathbf{x})), \\
%     % \mathcal{T}(\mathbf{x}) &= \textrm{ReLU}(1-\textrm{inf} \cdot \mathcal{T}_2(\mathbf{x})), \\
%     \mathcal{S}(\mathcal{F}(\mathbf{x})) &= \mathcal{T}_2(\mathbf{x}) \times \mathcal{F}(\mathbf{x})
% \end{align*}
\begin{equation*}
    t_\epsilon (\mathbf{v}) = 1 - \textrm{ReLU}(1-L \max\limits_{1 \le i \le |\mathbf{v}|}\textrm{ReLU}(|\mathbf{v}_i| - \epsilon))
\end{equation*}

\noindent where $L$ refers to a very large positive constant (e.g., $1e5$ in our experiments). Then, $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{v}))$ has the following form:
\begin{equation*}
    % t = 1 - \textrm{ReLU}(1-\textrm{inf} \cdot \max\limits_{i \in \{1, ..., n\}}\textrm{ReLU}(|\mathcal{F}(\mathbf{x})_i| - \epsilon)), \\
    % \mathcal{T}(\mathbf{x}) &= \textrm{ReLU}(1-\textrm{inf} \cdot \mathcal{T}_2(\mathbf{x})), \\
    \mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x})) = t_\epsilon (\mathcal{F}(\mathbf{x})) \mathcal{F}(\mathbf{x})
\end{equation*}

Recall that each layer of Transformer consists of two residual blocks, namely, the self-attention sub-layer and the position-wise FFN sub-layer. We apply the $\epsilon$ network directly to the residual block in the FFN sub-layer, i.e., 
% \todo[color=green]{Split this subsection into original attention and multi-head residual variant. Move the former to the preliminary subsection.}
% \todo[color=green]{This S is in fact the F not the S in the eq on line 253. Better rename S.}
\begin{align*}
    \mathcal{H}_\textrm{FFN}(\mathbf{x}) = \mathcal{S}_{\epsilon_\textrm{FFN}}(\textrm{FFN}(\mathbf{x})) + \mathbf{x},
\end{align*}

\noindent When applying it to the attention sub-layer, we employ a modified attention architecture by placing a residual connection to each single attention head, which allows us to prune any subset of attention heads, i.e., \todo{lzi: this is actually not true, there is only one residual connection link to the sum of epsilon(single attention head)}
% every single attention head in each attention sub-layer so that we can prune individual attention head:
\begin{align*}
    \mathcal{H}_\textrm{ATT}(\mathbf{x}) = \sum_{i=1}^A \mathcal{S}_{\epsilon_\textrm{ATT}}(\textrm{head}_i W^O_i) + \mathbf{x}
\end{align*}

\noindent Here, $W^O_i$ is the output weight assign to the $i$-th attention head, i.e., $W^O=[W^O_I, W^O_2, ..., W^O_A]$. If $\mathcal{S}_{\epsilon_\textrm{ATT}}(\textrm{head}_i W^O_i) = 0$, this means that the $i$-th attention head does not contribute to the output of the attention layer and thus could be pruned out.

In our experiment, we set different values to $\epsilon_\textrm{ATT}$ and $\epsilon_\textrm{FFN}$, since the absolute outputs of attention and FFN layers lay in different scalars, as illustrated in Figure \ref{fig:output-distribution}.

% Based on the above definitions, our $\epsilon$-Transformer could be defined as $\mathcal{H}(\mathbf{x}) = \mathcal{S}(\mathcal{F}(\mathbf{x})) + \mathbf{x}$, where $\mathcal{F}(\mathbf{x})$ could be $\textrm{Multi-head}(Q, K, V)$ or $\textrm{FFN}(\mathbf{x})$.

\begin{figure*}[tb]
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/att_output_distibution.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/ffn_output_distibution.pdf}
    \end{minipage}
    \\
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/att_output_distibution_norm=2.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
    \centering
        \includegraphics[width=1.0\textwidth]{images/distribution/new/ffn_output_distibution_norm=2.pdf}
    \end{minipage}
    \caption{Distribution of the max absolute value of the attention/FFN outputs on the Stanford Sentiment Treebank (SST) training set, based on model BERT$_\textrm{BASE}$ (w/o SN) and spectral normalized BERT$_\textrm{BASE}$ (w/ SN). For attention layers, different heads are plotted separately but with the same color in the same layer for clarity.}
    \label{fig:output-distribution}
\end{figure*}

\subsection{Spectral Normalization}
\label{sec:sepctral-normalization}
% motivation of normalizing the weight

% As discussed in Section \ref{sec:identity_mapping}, the sparse-inducing mechanism $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x}))$ takes effect when $|\mathcal{F}(\mathbf{x})_i|<\epsilon$. Clearly, the effectiveness of such a approach relies on a key assumption: within each layer, the statistical distribution of the function norms of the unimportant and the important residual mappings $P(|\mathcal{F}_{\texttt{unimp}}(\mathbf{x})_i|) \, v.s. \, P(|\mathcal{F}_{\texttt{imp}}(\mathbf{x})_i|)$ can be well-separated by $\epsilon$, such that there exists an $\epsilon$ so that the probabilities $P(|\mathcal{F}_{\texttt{unimp}}(\mathbf{x})_i|<\epsilon)$ and $P(|\mathcal{F}_{\texttt{unimp}}(\mathbf{x})_i|>\epsilon)$ are both close to 1. Unfortunately, such separation was not easily observed in the function norm distribution of a standard pre-trained BERT model. For example, in Figure \ref{fig:output-distribution} (Top row), we observe that the function norm distribution for the attention head outputs tend to be densely clustered within the range $[0, 2]$. On the other hand, the norm distribution for the FFN layer outputs varies widely within the range $[0, 1000]$.

In its originally proposal, the sparse-inducing function $\mathcal{S}_\epsilon(\mathcal{F}(\mathbf{x}))$ were found to work well for randomly initialized neural network, where the initial weight matrix of the nonlinear mappings for all layers were distributed within a consistent range, and thus facilitates a natural separation between the function norms $|\mathcal{F}|$ of the important and unimportant nonlinear mappings in the residual blocks during training \citep{yu2018learning}. This is, however, not the case for the weight distribution for a pre-trainined model like BERT, where the weight distributions between different layers have already diverged during pre-training, likely to due to the specialization of layer functionalities under the masked language modeling (MLM) training \citep{tenney2019bert}. Indeed, in our preliminary experiments, we observed that the proposed identity-inducing prior $\epsilon$ is not effective for a BERT model initialized from a classic pre-training checkpoint. Empirically, as shown in Figure \ref{tab:performance-on-different-norm}, we found the distribution of the function norms $P(|F(\mathbf{x})_i|)$ for the attention layers to be densely clustered within a small range ($(0, 2)$) and with no clear separation between the function norm for the important and unimportant nonlinear residual mappings. On the other hand, the norm distributions for different FFN layers were found to vary wildly, creating challenges for selecting a proper set of $\epsilon$'s in practice.

% In our preliminary experiments, we observed that when applying the defined $\epsilon$-Transformer\todo{another new term? eps-ResNet vs eps-Transformer vs eps network? Maybe add in the previous subsection, we define eps-Transformer as such and such.} to BERT, the distribution of $|\mathcal{F}(\mathbf{x})|$ is of low sparsity\todo{what is sparsity of a distribution? maybe "screwed"?} and the maximum of $|\mathcal{F}(\mathbf{x})|$ for the FFN sub-layer is usually very large, resulting in the difficulty for us to choose a proper set of $\epsilon$.\todo{it's not very clear why these phenomena made it hard to choose eps. shouldn't varied max and distribution across sublayers, layers, and tasks make it hard?}

The above observations motivate us to identify an effective method to stabilize the norm distributions of the BERT model layers. In this work, we consider \textit{Spectral Normalization} (SN), an approach that directly control the Lipschitz norm of a nonlinear mapping $\mathcal{F}$ by regularizing the spectral behavior of its weight matrices \citep{miyato2018spectral}. 

Specifically, for a weight matrix $W$, its spectral norm $\lambda(W)$ is defined as its largest singular value:
\begin{align*}
    \lambda(W) = 
    %\underset{\mathcal{F}_{k-1}}{\textrm{sup}}\sigma(\nabla\mathcal{F}_{k}) = 
    \underset{x\neq0}{\textrm{max}}\frac{||W\mathbf{x}||_2}{||\mathbf{x}||_2}.
\end{align*}
We say a function $\mathcal{F}$ is $L$-Lipschitz if $|\mathcal{F}(x_1)-\mathcal{F}(x_2)|/||x_1 - x_2|| \leq L$, for all $x_1$, $x_2$, and we call the smallest possible $L$ the Lipschitz norm of $\mathcal{F}$, denoted as $|\mathcal{F}|_{Lip}$. 
%In other words, small changes in the input of the function causes corresponding small changes in the magnitude of its gradients. From its definition, the Lipschitz constant of a given layer $k$ of a neural network, whose activations are given by 
Consequently, for a neural network mapping $\mathcal{F}(\mathbf{x}) = \sigma(W\mathbf{x} + b)$ with an contractive activation function $\sigma$,
%\todo{unparsable sentence}
%Similar to other weight normalization methods, spectral normalization normalizes the weight $W$ by the spectral norm (or $L_2$ matric norm), denoted as $\sigma(W)$\todo{sigma is redefined}.
%\noindent which is essentially the largest singular value of the matrix $W$. In our case, spectral normalization guarantees the norm of the function $\mathcal{F}(\mathbf{x})$ resides in a finite region upper bounded by
its Lipschitz norm is upper-bounded by $\lambda(W)$ \citep{miyato2018spectral}:
\begin{equation*}
    |\mathcal{F}|_{Lip} = |\sigma(W \mathbf{x} + b)|_{Lip} \leq |W \mathbf{x} + b|_{Lip} \leq \lambda(W).
\end{equation*}
For BERT models, since the layer input $\mathbf{x}$ follows a  distribution of zero mean and unit variance due to layer normalization \cite{ba2016layer}, a nonlinear mapping's $L_1$ norm $|\mathcal{F}|$ is roughly proportional to its Lipschitz norm $|\mathcal{F}|_{Lip}$, which is controlled by $\lambda(W)$.

Therefore, we are able to have a better control of the maximum of $|\mathcal{F}(\mathbf{x})|$ for identifying a good $\epsilon$. Furthermore, the regularization is achieved by that the layer weights are simply divided by their corresponding spectral norm in SN, i.e. $\hat{W} = W / \hat{\lambda}(W)$, adding no additional trainable  parameter to the original model.

We applied SN to both pre-training and fine-tuning of the BERT model, and on the weights in both the attention and the FFN layers. As shown in Table \ref{tab:performance-on-different-norm}, adding SN to a BERT$_\textrm{BASE}$ model resulted in improved pre-training performance and competitive fine-tuning performance when compared to the original BERT$_\textrm{BASE}$ without SN. To illustrate the effect of SN on the function norms of the BERT model, we plot $|\mathcal{F}(\mathbf{x})|$ for the training set of the Stanford Sentiment Treebank in Figure \ref{fig:output-distribution}. As shown, after SN, the norm distribution $P(|\mathcal{F}_k(\mathbf{x})|)$ between the important and the unimportant nonlinear mappings shows a better separation (Figure \ref{fig:output-distribution}, bottom left), the norms distribution for the FFN layers are now stabilized within a much smaller range (Figure \ref{fig:output-distribution}, bottom right). More examples could be found in the supplementary materials.
%\textbf{Strict weight normalization can sacrifice the expressive power of the network. This could addressed by using less strict Lipschitz constraint $\sigma(W)$, as shown in Table \ref{tab:performance-on-different-norm}.}
% \todo[color=white]{\jzl{this discussion seem to contradict with the statement in the previous paragraph. It might be good to put this discussion to a less prominent place. and mention that strict weight normalization can harm the expressive power of the network due to the existence of the non-gradient-norm preserving activation function, as well as the other regularization mechanisms in the model which scales down the Lipschitz constant in unexpected ways. (you can cite and check out first paragraph of this paper: https://arxiv.org/pdf/1811.05381.pdf)}}
% As excessive normalization can do harm to the model's prediction performance, we found that relatively loosing the target Lipschitz constraint $\sigma(W)$ to some value larger than 1 could have rather negligible or even positive impact on the training process compared to the standard Transformer, as shown in Table \ref{tab:performance-on-different-norm}.

\begin{table}[tb]
    \centering\scalebox{0.8}{
    \begin{tabular}{lcccccc}
    \hline
        \textbf{SN}                  & \textbf{MLM} & \textbf{SST-2} & \textbf{QQP} & \textbf{MRPC} & \textbf{QNLI} & \textbf{MNLI}\\\hline
        w/o                & 71.93       & 92.7        & 90.6        & 90.9         & 91.6         & 84.7           \\
        % BERT$_\textrm{BASE}$ ($\sigma(W)=1$) & 70.72       & 90.4        & 89.0        & 89.2         & 89.0         & 80.6           \\
        % BERT$_\textrm{BASE}$ ($\sigma(W)=2$) & 73.43       & 91.3        & 90.1        & 90.3         & 91.5         & 84.0           \\
        w/ & 74.16       & 91.9        & 90.1        & 90.8         & 91.6         & 85.1           \\
    \hline
    \end{tabular}}
    \caption{Evaluate the performance of BERT$_\textrm{BASE}$ (w/o SN) and the spectral normalized BERT$_\textrm{BASE}$ (w/ SN, using $\lambda(W)=5$), respectively masked language modeling accuracy on pre-training data and accuracy of fine-tuning on 5 natural language understanding tasks (details could be found in Section \ref{sec:datasets}).
    }
    \label{tab:performance-on-different-norm}
\end{table}


% \todo{add an eq between eps and sigma}
% \todo{How to explain that spectral normalization could improve the sparsity of the distribution}
% \todo[color=green ]{jzl: Should we show $\sigma(W)=5$ results instead? Or just change image title to "with spectral regularization"}

% \subsection{Distillation Objective}

% \paragraph{Traditional Distillation} 
% Basically, for training set $\mathcal{D} = {(x^1, y^1), ..., (x^i, y^i))}$, let the output of student model with parameters $\theta$ on the input $x$ be $f(x, \theta)$, and the corresponding output of a well-trained teacher model with parameters $\theta'$ be $f(x, \theta')$. The model distillation trains $\theta$ to minimize the loss on the training set:

% \begin{equation*}
%     \mathcal{L}(\theta)=\sum_{x^i, y^i \in \mathcal{D}}\ell(f(x^i, \theta'), f(x^i, \theta))
% \end{equation*}

% where for classification tasks $\ell$ is the cross entropy loss.

% Several works has proven that we can actually set up the teacher and student have the same neural architecture and model size, but surprisingly the student is able to surpass the teacher's accuracy, which is called Born-Again \cite{furlanello2018born, clark2019bam}. This could be explained by that, distillation is effective because the teacher's output distribution over classes provides more training signal than simple one-hot labels. Given that fact, we start from the student $\epsilon$-Transformer model with the same size as the teacher standard Transformer model. As learning the identity mapping within residual block of the attention and feed forward network, the student will automatically discard the redundant layers.

% \paragraph{Teacher Annealing} In knowledge distillation, the student is trained to imitate the teacher. This raises the concern that the student may be limited bu the teacher's performance and not be able to substantially outperform the teacher. To address this, we use \textit{teacher annealing} proposed by \cite{clark2019bam}, which mixes the teacher prediction with the gold label during training, so the loss function becomes

% \begin{equation*}
%     \mathcal{L}(\theta)=\sum_{x^i, y^i \in \mathcal{D}}\ell(\lambda f(x^i, \theta') + (1-\lambda)y^i , f(x^i, \theta))
% \end{equation*}

% where $\lambda$ refers to how much weight to put on distill targets compared to gold-standard labels.
\begin{figure*}[tb]
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/sst.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/qqp.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \includegraphics[width=5.5cm]{images/performance/mrpc.pdf}
    \end{minipage}%
    \\
    \begin{minipage}[t]{0.5\textwidth}
        \includegraphics[width=5.5cm, right]{images/performance/qnli.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \includegraphics[width=5.5cm, left]{images/performance/mnli.pdf}
    \end{minipage}
\caption{Evolution of performance when separately pruning attention heads (ATT) and FFN layers (FFN), and joint pruning ATT and FFN (Joint) on 5 GLUE dev sets. * means applying spectral normalization. The percentage pruned (x-axis) is calculated based on the parameters of attention and FFN sub-layers as the full set (excluding embedding, pooler and classifier layers).}
\label{fig:results}
\end{figure*}

\subsection{Iterative Pruning}
The choice of $\epsilon_\textrm{ATT}$ and $\epsilon_\textrm{FFN}$ can be regulated by some prior distribution and optimized during training. We use a simple pruning method that greedily and iteratively prunes away attention heads and FFN layers, which can avoid impractical combinatorial search given the number of attention heads and the time it takes to evaluate each model. The method employs a three-step process: 

(1) Evaluate the output distribution at each iteration to give a heuristics for the selection of $\epsilon$. As $\epsilon$ satisfies a nice monotonicity property --- larger value leads to higher compression, we could start from a relatively low $\epsilon$ and gradually increase it at each iteration. \todo{there should be a problem, since we try to restrict the magnitude but turns out choose $\epsilon$ based on empirical distribution}

(2) Top-down training: train the full-size model with the selected $\epsilon$. Prune the low-weight connections by removing the weights below a threshold. When a residual block produces negligible response, the $\epsilon$ function will start producing $0$ outputs. As a result, the weights in this block will stop contributing to the cross-entropy term. Consequently, the gradients will only based on the regularization term and lead to weight collapse.% It is noted that spectral normalization will help the weight go to zeros more quickly since the largest singular value of the weight has been restricted.

(3) Retrain the compressed model to learn the final weight for the remaining sparse connections. This is critical --- if the pruned network is used without retraining, accuracy is significantly impacted. Also, during retraining, it is better to retain the weights from the initial training phase for the connections that survived pruning than it is to re-initialize them \cite{han2015learning}.
% \todo{Should this subsection be moved to the method section above? +1 to move to method section nhua. Besides "than it is to re-initialize them"?}

==> sections/old/04.experiments.tex <==
\begin{table*}[tb]
    \centering
    \scalebox{0.7}{
    \begin{tabular}{lrccccc}
    \hline
        \textbf{Model}                            & \textbf{FLOPS} & \textbf{ SST-2$_{acc}$} & \textbf{QQP$_{acc}$} & \textbf{MRPC$_{F_1}$} & \textbf{QNLI$_{acc}$} & \textbf{MNLI-mm$_{acc}$}\\\hline
        BERT$_\textrm{BASE}$                      & 22.5B          & \ \ -0.0\%/92.7        & \ \ -0.0\%/90.6       & \ \ -0.0\%/90.9        & \ \ -0.0\%/91.6        & \ \ -0.0\%/84.7 \\
        TinyBERT$_6$ w/o DA \cite{jiao2019tinybert} & 1.2B         & -                      & -                     & -50.0\%/86.0           & -                      & \textbf{-50.0\%/84.4}\\
        DistillBERT$_6$ \cite{sanh2019distilbert} & 11.3B          & -50.0\%/91.3           & -50.0\%/88.5          & -50.0\%/87.5           & -50.0\%/89.2           & -50.0\%/82.2 \\
        BERT-PKD$_6$ \cite{sun2019patient}        & 11.3B          & -50.0\%/91.5           & \textbf{-50.0\%/88.9}          & -50.0\%/86.2           & -50.0\%/89.0           & -50.0\%/81.0 \\
        BERT-PKD$_3$ \cite{sun2019patient}        & 7.6B           & -75.0\%/87.5           & -75.0\%/87.8          & -75.0\%/80.7           & -75.0\%/84.7           & -75.0\%/76.3 \\
        \hline
        % MobileBERT \cite{sun2020mobilebert} *, $\dagger$   & 76.8\%/91.7           & 76.8\%/88.3          & 76.8\%/87.5           & 76.8\%/91.5           & 76.8\%/83.4 \\
        % RPP-BERT$_\textrm{LARGE}$ \cite{guo2019reweighted}& -64.1\%/92.4           & -64.1\%/89.2          & -64.1\%/81.9           & -64.1\%/88.0           & -64.1\%/81.8 \\\hline
        % $\epsilon$-BERT                       & -30.0\%/91.3                 & -38.7\%/89.5                & -39.7\%/89.9                 & -26.1\%/90.8                 & -32.3\%/83.5\\
        FLOP \cite{wang2019structured}           & 15B             & -35.0\%/92.1           & -                     & -35.0\%/88.6           & -35.0\%/89.0           & -           \\
        MvP \cite{sanh2020movement} $\dagger$    & N/A             & -                      & -97.0\%/89.2          & -                      & -                      & -97.0\%/79.7\\\hline\hline
        $\epsilon$-BERT (ours, w/ SN)          & 13.2 - 14.5B    & \textbf{-50.0\%/91.8}           & \textbf{-50.0\%/88.9}         & \textbf{-50.0\%/88.1}           & \textbf{-50.0\%/89.5}           & -50.0\%/82.8\\
        $\epsilon$-BERT (ours, w/ SN)          & 8.3 - 9.1B      & -75.0\%/88.4           & -75.0\%/87.8          & -75.0\%/81.2           & -75.0\%/84.6           & -75.0\%/78.3\\\hline
        $\epsilon$-BERT (ours, w/o SN)                          & 16.8 - 18.2B    & -30.0\%/91.3           & -38.7\%/89.5          & -39.7\%/89.9           & -26.1\%/90.8           & -32.3\%/83.5\\
        % $\epsilon$-BERT ($\sigma(W)=2$)        &                 & -45.3\%/91.3           & -38.6\%/89.7          & -53.3\%/89.8           & -26.7\%/90.5           & -31.4\%/83.6\\
        $\epsilon$-BERT (ours, w/ SN)          & 13.4 - 16.1B    & -56.7\%/91.7           & -40.7\%/89.7          & -46.7\%/89.9           & -36.0\%/90.7           & -39.3\%/83.9\\
        \hline
    \end{tabular}}
    \caption{The compression results including model efficiency (percentage of reduced parameters) and performance from the GLUE dev results, and the MNLI result is evaluate for mismatched-accuracy (MNLI-mm). BERT$_\textrm{BASE}$ indicates the results of the fine-tuned BERT$_\textrm{BASE}$ in our implementation. The number of model parameters includes the attention and FFN sub-layers but excludes the embedding, pooler and classifier layers. The bold numbers indicate the best performance for keeping 50\% of the parameters respectively. $\dagger$ means unstructured pruning, which could not speed up the inference in practice.}% The RPP-BERT was trained based on BERT$_\textrm{LARGE}$, which means it can be unfair to make a direct comparison.} %* means part of the pruned parameters comes from the embedding layers, and $\dagger$ means the compression is task-agnostic.}
    \label{tab:best-architecture}
\end{table*}

\todo{lzi: is the last two lines of the table necessary? since it could actually be read from Figure 3.}
\section{Experiments}
% \todo[color=green]{Figure 1 and table 1 are not referenced in the content.}
% \todo[color=green]{Increase fonts for all figures.}

\subsection{Experimental Settings}
In the experiments, we apply the same architecture and the base settings from the original BERT$_\textrm{BASE}$ \cite{devlin2018bert}, and fine-tune each task independently. More details could be found in supplementary materials.
\todo{weight based pruning baselines?}

% The key hyperparameters are the thresholds $\epsilon_{ATT}$ and $\epsilon_{FFN}$, where we apply an iterative pruning as discussed in the next subsection.

\subsection{Datasets}
\label{sec:datasets}
For pre-training, we use the same data as BERT, which consists of 3.3 Billion tokens from Wikipedia and BooksCorpus \citep{zhu2015aligning}. 
For fine-tuning tasks, we conduct experiments on the subset of the General Language Understanding Evaluation (GLUE) Benchmark \citep{wang2018glue}, classified into three categories: (1) sentiment analysis: Stanford Sentiment Treebank (SST, \cite{socher2013recursive}); (2) paraphrasing: Quora Question Pairs (QQP, \cite{chen2018quora}), Microsoft Research Paraphrase Corpus (MRPC, \cite{dolan2005automatically}); (3) natural language inference: Question Natural Language Inference (QNLI, \cite{chen2018quora}), Multi-genre Natural Language Inference (MNLI, \cite{williams2017broad}). The reason for choosing this subset is that we found the variance in performance for those tasks lower than the other GLUE tasks. Further details about those tasks could be found in supplementary materials.
% \todo[color=green]{Reasons for the subset use like Dan said.}

\subsection{Results}
We compare the pruning results on non-normalized and normalized BERT models on the 5 GLUE tasks, as shown in Figure \ref{fig:results}, which includes separate pruning for attention heads and FFN sub-layers and joint pruning for both sub-modules. The results demonstrate the advantage of using spectral normalization.\textbf{ To put it all together, in Table \ref{tab:best-architecture}, we further show the simplest architecture we could get when allowed at most 1\% in terms of  performance degradation. This also means that further slight pruning will have noticeable impact on the final results. }
%where we first trained the pruning of attention heads and FFN layers separately to get the full evolution of the performance during the training process.

% Finally, to put it all together, we dynamically train the pruning of both attention heads and FFN sub-layers. The final $\epsilon$-BERT allows us to choose the simplest architecture corresponding to any negligible results, and in Table \ref{tab:best-architecture}, we further show the simplest architecture we could get when allowed at most 1\% in terms of  performance degradation. This also means that further slight pruning will have noticeable impact on the final results. 

We also list other compression methods in the table for comparison while most of them are of knowledge distillation and have a pre-defined fixed size of the compressed model.
Our methods provide the flexibility to choose the best architecture and take the advantage of finding the inflection point during pruning, while compared with other pruning methods we could practically speed up the inference time since we use a structured pruning.
\footnote{TinyBERT \cite{jiao2019tinybert} utilizes data augmentation (DA) to improve the distillation results, which makes it unfair to have a direct comparison, so here we only listed their results without DA. As for the unstructured pruning in MvP \cite{sanh2020movement}, current hardware does not support optimized inference for the sparse model so it is actually hard to put it in practice. We do not list the results in \citet{guo2019reweighted, gordon2020compressing} since they show the results in scatter plots instead of the exact numbers, and similarly they are of unstructured pruning.}%i.e, though some models save more parameters, their results are far below the original BERT, without noticing that: (1) actually slightly adding more parameters could keep almost the same performance, (2) sometimes compressing further still does no harm, and (3) different tasks need different model size. Furthermore, unlike other models, $\epsilon$-BERT does not need to transfer the knowledge of each layer from the teacher model or doing data augmentation to provide more task-specific data.

==> sections/old/05.ablation_study.tex <==
\begin{figure*}[tb]
    \centering
    \begin{tabular}{p{0.005\textwidth}p{0.28\textwidth}p{0.28\textwidth}p{0.28\textwidth}}
            & \multicolumn{1}{c}{\ \ \ \ \ SST}   & \multicolumn{1}{c}{\ \ \ \ \ MRPC} &\multicolumn{1}{c}{\ \ \ \ \ MNLI} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 16.67\%} &  \includegraphics[width=0.3\textwidth]{images/ablation/sst/sst_iter1.pdf}    & \includegraphics[width=0.3\textwidth]{images/ablation/mrpc/mrpc_iter1.pdf} & \includegraphics[width=0.3\textwidth]{images/ablation/mnli/mnli_iter1.pdf} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 33.33\%} &  \includegraphics[width=0.3\textwidth]{images/ablation/sst/sst_iter2.pdf}    & \includegraphics[width=0.3\textwidth]{images/ablation/mrpc/mrpc_iter2.pdf} & \includegraphics[width=0.3\textwidth]{images/ablation/mnli/mnli_iter2.pdf} \\
     \rotatebox{90}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 50.00\%} &  \includegraphics[width=0.3\textwidth]{images/ablation/sst/sst_iter3.pdf}    & \includegraphics[width=0.3\textwidth]{images/ablation/mrpc/mrpc_iter3.pdf} & \includegraphics[width=0.3\textwidth]{images/ablation/mnli/mnli_iter3.pdf}
    \end{tabular}
    \caption{Faded map of attention heads and FFN layers during pruning on task SST-2, MRPC and MNLI dev sets. Color white indicates that this attention head or FFN layer has been entirely pruned out. The left column shows the percentage pruned, and \texttt{mean} is the mean of attention heads of each layers.}
    \label{fig:heatmap}
\end{figure*}

\begin{figure}[tb]
    \centering
    \includegraphics[width=6cm]{images/ablation/ablation.pdf}
    \caption{Evolution of accuracy on the dev set of SST-2 for (1) pruning the whole attention layers (HA); (2) pruning single attention heads (MHA); (3) layer pruning means pruning the whole layer (Layer pruning) and (4) pruning the attention and FFN sub-layers separately (Split pruning).}
    \label{fig:abaltion}
\end{figure}

\section{Ablation Study}
In this section, we investigate the contribution of: (1) single attention head pruning, and (2) split pruning for attention heads and FFN sub-layers.

\paragraph{Single Head Attention Pruning}

Multi-head self-attention is a key component of Transformer, where each attention head potentially focusing on different parts of the inputs. The analysis of multi-head attention and its importance is challenging. Previous analysis of multi-head attention considered the average of attention weights over all heads at given position or focused only on the maximum attention weights \cite{voita2018context, tang2018analysis}, or explicitly takes into account the varying importance of different heads \cite{voita2019analyzing}. Moreover, \citet{michel2019sixteen} has proved that a large percentage of attention heads can be removed at test time without significantly impacting performance, but they mainly discussed the case on machine translation and NLI tasks, and it is still unknown whether attention heads play consistent and interpretable roles when trained on different downstream tasks.

To probe this question, we pick one task from the sentiment analysis, paraphrasing and natural language inference respectively, plot the pruned attention heads during training and show the dynamic process in Figure \ref{fig:heatmap}, where we can find that though for different tasks, the distribution of important attention heads are similar, as reflected in the mean of each attention layer, but the exact pruned attention heads are actually different. This also indicates that splitting the pruning for attention heads could have more flexibility for the model to find an optimal architecture.

\paragraph{Separate Pruning for Attention and FFN}
% To allow the different attention heads to interact with each other, the Transformer model applies a non-linear feed-forward network over the multi-head attention's output at each layer \cite{vaswani2017attention}. 
Decoupling and then individually studying the self-attention and the FFN sub-layers is important for understanding the progressive improvement they provide.
As can be observed from Figure \ref{fig:results}, for most of the tasks, the negative effect brought by pruning FFN layers are way more significant than attention layers, indicating that the compression technique for the Transformer model is usually highly effective on the attention layers \cite{voita2018context, michel2019sixteen}, but may be less successful on the fully connected layers \cite{ganesh2020compressing}. In Figure \ref{fig:heatmap}, similar to attention heads, we further plot the faded map of FFN layers, and find that, certain FFN sub-layers might be more amenable to compression, even if the corresponding self-attention sub-unit is not. For example, in all the tasks, the FFN layer near the ends of input or output are more likely to be pruned, while this is not the case for the corresponding self-attention layers.

Finally, to valid the advantage of the single head attention pruning and split pruning for attention/FFN, we further show the evolution of performance for single head attention pruning (HA), multi-head attention pruning (MHA), separate attention/FFN pruning, and whole layer pruning respectively in Figure \ref{fig:abaltion}.

% The compression technique for the Transformer model is usually highly effective on the attention layers \cite{voita2018context, michel2019sixteen}, but may be less successful on the fully connected layers, while clearly the latter part consuming the most memory and executing the highest number of Floating Point Operations Per Second (FLOPS).


